Reinforcement Learning for Scalable and Trustworthy Intelligent Systems

Reinforcement learning has become a powerful paradigm for improving the capability of intelligent systems, but its practical deployment faces two central challenges. First, reinforcement learning must scale efficiently in distributed environments where communication bandwidth is limited and computation is heterogeneous across agents. Second, as reinforcement learning is increasingly used in post-training large language models and autonomous agents, the optimized policies must also be aligned with human preferences and satisfy safety requirements such as privacy-aware information disclosure. This dissertation addresses both challenges through four complementary contributions spanning federated optimization, preference alignment, and contextual safety. The first part of the dissertation studies scalable reinforcement learning in federated settings. The second part of the dissertation studies trustworthy reinforcement learning for large language models. Together, these contributions advance reinforcement learning along two complementary dimensions. On the one hand, they make reinforcement learning more scalable through communication-efficient and asynchronous federated optimization. On the other hand, they make reinforcement learning more trustworthy by improving alignment with human preferences and by reducing contextually inappropriate information disclosure in language-based intelligent systems. As a whole, this dissertation argues that the next generation of intelligent systems will require both efficient optimization and trustworthy behavior, and that reinforcement learning provides a unifying framework for addressing both goals.

==> ap-defining-commands.tex <==
\ProvidesFile{ap-defining-commands.tex}[2022-10-05 defining commands appendix]

\begin{VerbatimOut}{z.out}
\chapter{DEFINING COMMANDS}

The next paragraph demonstrates how to define and use a command.

\renewcommand{\t}[2]
{% The "{%" hides the space caused by the newline.  LaTeX ignores leading spaces on a line.
  Editors recommend that a #1 should never be
  followed by a #2 without some intervening text.
}

\t{chapter title}{section heading}
I suggest writing for readers.
Break the rules if necessary.
\end{VerbatimOut}

\MyIO


==> ap-electrical-engineering.tex <==
\ProvidesFile{ap-electrical-engineering.tex}[2022-10-05 electrical engineering appendix]

\begin{VerbatimOut}{z.out}
\chapter{ELECTRICAL ENGINEERING}
\ix{electrical engineering//Electrical Engineering appendix}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}


\section{Amplifiers}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
This \qty{18}{\W} MOSFET amplifier
with npn transistor was done by Ram\'on Jaramillo
\cite{jaramillo}.
\ix{Jaramillo, Ram\'on}
This example make uses the \CircuiTikZLogo\index{\CircuiTikZLogo}
\cite{redaelli2021}
\ix{Redaelli, Massimo A.}%
and siunitx packages.

\begin{tikzpicture}[scale=2]
  \draw[color=black, thick]
    (0,0) to [short,o-] (6,0){} % Baseline for connection to ground
    % Input and ground
    (0,1) node[]{\large{\textbf{INPUT}}}
    % Connection of passive components
    (5,0) node[ground]{} node[circ](4.5,0){}
    (0,2) to [cC, l=$C_1$, o-] (0.5,2)
    to [R,l=$R_1$,](1.5,2)
    to node[short]{}(2.6,2)
    (1.5,2) to [C, l=$C_2$, *-] (1.5,3) -| (5,3)
    (2.2,2) to [R, l=$R_2$, *-*] (2.2,3)
    (2.2,3) to [cC, l=$C_3$, *-] (2.2,5) -| (3,5)
    % Transistor Bipolar Q1
    (3,0) to [R,l=$R_5$,-*] (3,1.5)
    to [Tnpn,n=npn1] (3,2.5)
    (npn1.E) node[right=3mm, above=5mm]{$Q_1$} % Labelling the NPN transistor
    (4,0) to [cC, l_=$C_4$, *-] (4, 1.5)--(3,1.5)
    (2.2,0) to [vR, l=$R_3$, *-*] (2.2,2)
    (3,2.5) to node[short]{}(3,3)
    (3,5) to [pR, n=pot1, l_=$R_4$, *-] (3,3)
    (3,5) to [R, l=$R_6$, *-] (5,5)
    to [short,*-o](5,5.5) node[right]{$V_S=40 V$}
    % Mosfet Transistors
    (5,3) to [Tnigfetd,n=mos1] (5,5)
    (mos1.B) node[anchor=west]{$Q_2$} % Labelling MOSFET Q2 Transistor
    (pot1.wiper) to [R, l=$R_7$] (4.5,4) -| (mos1.G)
    (5,1.5) to [Tpigfetd,n=mos2] (5,2.5)
    (5,0) to (mos2.S)
    (3,2.5) to [R, l=$R_8$, *-] (4.5,2.5)
    -| (mos2.G)
    (mos2.B) node[anchor=west]{$Q_3$} % Labelling MOSFET Q3 Transistor
    % Output
    (6,3) to [cC, l=$C_5$,-*](5,3)
    (6,3) to [short,-o] (6,2){}
    (mos1.S)--(mos2.D)
    (6,0) to [short,-o] (6,1){} node[above=7mm]{\large{\textbf{SPEAKER}}}
    ;
\end{tikzpicture}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}


\section{Kalman Filter System Model}

This Kalman filter system model was done by Burkart Lingner
\cite{lingner2010}.
\ix{Lingner, Burkart}

% An example using TikZ/PGF 2.00
%
% Features: Decorations, Fit, Layers, Matrices, Styles
% Tags: Block diagrams, Diagrams
% Technical area: Electrical engineering

%%%% \documentclass[a4paper,10pt]{article}
%%%% 
%%%% \usepackage[english]{babel}
%%%% \usepackage[T1]{fontenc}
%%%% \usepackage[ansinew]{inputenc}
%%%% 
%%%% \usepackage{lmodern}	% font definition
%%%% \usepackage{amsmath}	% math fonts
%%%% \usepackage{amsthm}
%%%% \usepackage{amsfonts}
%%%% 
%%%% \usepackage{tikz}
%%%% 
%%%% %%%<
%%%% \usepackage{verbatim}
%%%% \usepackage[active,tightpage]{preview}
%%%% \PreviewEnvironment{tikzpicture}
%%%% \setlength\PreviewBorder{5pt}%
%%%% %%%>
%%%% 
%%%% \begin{comment}
%%%% :Title: Kalman Filter System Model
%%%% :Slug: kalman-filter
%%%% :Author: Burkart Lingner
%%%% 
%%%% This is the system model of the (linear) Kalman filter. 
%%%% 
%%%% \end{comment}
%%%% 
%%%% 

\begin{figure}[htbp]
\caption{Kalman filter system model}
\centering
% The state vector is represented by a blue circle.
% "minimum size" makes sure all circles have the same size
% independently of their contents.
\tikzstyle{state}=[circle,
                                    thick,
                                    minimum size=1.2cm,
                                    draw=blue!80,
                                    fill=blue!20]

% The measurement vector is represented by an orange circle.
\tikzstyle{measurement}=[circle,
                                                thick,
                                                minimum size=1.2cm,
                                                draw=orange!80,
                                                fill=orange!25]

% The control input vector is represented by a purple circle.
\tikzstyle{input}=[circle,
                                    thick,
                                    minimum size=1.2cm,
                                    draw=purple!80,
                                    fill=purple!20]

% The input, state transition, and measurement matrices
% are represented by gray squares.
% They have a smaller minimal size for aesthetic reasons.
\tikzstyle{matrx}=[rectangle,
                                    thick,
                                    minimum size=1cm,
                                    draw=gray!80,
                                    fill=gray!20]

% The system and measurement noise are represented by yellow
% circles with a "noisy" uneven circumference.
% This requires the TikZ library "decorations.pathmorphing".
\tikzstyle{noise}=[circle,
                                    thick,
                                    minimum size=1.2cm,
                                    draw=yellow!85!black,
                                    fill=yellow!40,
                                    decorate,
                                    decoration={random steps,
                                                            segment length=2pt,
                                                            amplitude=2pt}]

% Everything is drawn on underlying gray rectangles with
% rounded corners.
\tikzstyle{background}=[rectangle,
                                                fill=gray!10,
                                                inner sep=0.2cm,
                                                rounded corners=5mm]

\begin{tikzpicture}[>=latex,text height=1.5ex,text depth=0.25ex]
    % "text height" and "text depth" are required to vertically
    % align the labels with and without indices.
  
  % The various elements are conveniently placed using a matrix:
  \matrix[row sep=0.5cm,column sep=0.5cm] {
    % First line: Control input
    &
        \node (u_k-1) [input]{$\mathbf{u}_{k-1}$}; &
        &
        \node (u_k)   [input]{$\mathbf{u}_k$};     &
        &
        \node (u_k+1) [input]{$\mathbf{u}_{k+1}$}; &
        \\
        % Second line: System noise & input matrix
        \node (w_k-1) [noise] {$\mathbf{w}_{k-1}$}; &
        \node (B_k-1) [matrx] {$\mathbf{B}$};       &
        \node (w_k)   [noise] {$\mathbf{w}_k$};     &
        \node (B_k)   [matrx] {$\mathbf{B}$};       &
        \node (w_k+1) [noise] {$\mathbf{w}_{k+1}$}; &
        \node (B_k+1) [matrx] {$\mathbf{B}$};       &
        \\
        % Third line: State & state transition matrix
        \node (A_k-2)         {$\cdots$};           &
        \node (x_k-1) [state] {$\mathbf{x}_{k-1}$}; &
        \node (A_k-1) [matrx] {$\mathbf{A}$};       &
        \node (x_k)   [state] {$\mathbf{x}_k$};     &
        \node (A_k)   [matrx] {$\mathbf{A}$};       &
        \node (x_k+1) [state] {$\mathbf{x}_{k+1}$}; &
        \node (A_k+1)         {$\cdots$};           \\
        % Fourth line: Measurement noise & measurement matrix
        \node (v_k-1) [noise] {$\mathbf{v}_{k-1}$}; &
        \node (H_k-1) [matrx] {$\mathbf{H}$};       &
        \node (v_k)   [noise] {$\mathbf{v}_k$};     &
        \node (H_k)   [matrx] {$\mathbf{H}$};       &
        \node (v_k+1) [noise] {$\mathbf{v}_{k+1}$}; &
        \node (H_k+1) [matrx] {$\mathbf{H}$};       &
        \\
        % Fifth line: Measurement
        &
        \node (z_k-1) [measurement] {$\mathbf{z}_{k-1}$}; &
        &
        \node (z_k)   [measurement] {$\mathbf{z}_k$};     &
        &
        \node (z_k+1) [measurement] {$\mathbf{z}_{k+1}$}; &
        \\
    };
    
    % The diagram elements are now connected through arrows:
    \path[->]
        (A_k-2) edge[thick] (x_k-1)	% The main path between the
        (x_k-1) edge[thick] (A_k-1)	% states via the state
        (A_k-1) edge[thick] (x_k)		% transition matrices is
        (x_k)   edge[thick] (A_k)		% accentuated.
        (A_k)   edge[thick] (x_k+1)	% x -> A -> x -> A -> ...
        (x_k+1) edge[thick] (A_k+1)
        
        (x_k-1) edge (H_k-1)				% Output path x -> H -> z
        (H_k-1) edge (z_k-1)
        (x_k)   edge (H_k)
        (H_k)   edge (z_k)
        (x_k+1) edge (H_k+1)
        (H_k+1) edge (z_k+1)
        
        (v_k-1) edge (z_k-1)				% Output noise v -> z
        (v_k)   edge (z_k)
        (v_k+1) edge (z_k+1)
        
        (w_k-1) edge (x_k-1)				% System noise w -> x
        (w_k)   edge (x_k)
        (w_k+1) edge (x_k+1)
        
        (u_k-1) edge (B_k-1)				% Input path u -> B -> x
        (B_k-1) edge (x_k-1)
        (u_k)   edge (B_k)
        (B_k)   edge (x_k)
        (u_k+1) edge (B_k+1)
        (B_k+1) edge (x_k+1)
        ;
    
    % Now that the diagram has been drawn, background rectangles
    % can be fitted to its elements. This requires the TikZ
    % libraries "fit" and "background".
    % Control input and measurement are labeled. These labels have
    % not been translated to English as "Measurement" instead of
    % "Messung" would not look good due to it being too long a word.
    \begin{pgfonlayer}{background}
        \node [background,
                    fit=(u_k-1) (u_k+1),
                    label=left:Entrance:] {};
        \node [background,
                    fit=(w_k-1) (v_k-1) (A_k+1)] {};
        \node [background,
                    fit=(z_k-1) (z_k+1),
                    label=left:Measure:] {};
    \end{pgfonlayer}
\end{tikzpicture}

\end{figure}
\end{VerbatimOut}

\MyIO


==> ap-mathematics.tex <==
\ProvidesFile{ap-mathematics.tex}[2023-09-01 mathematics appendix]

\begin{VerbatimOut}{z.out}
\chapter{MATHEMATICS}
\ix{mathematics//Mathematics appendix}

\PurdueThesisLogo\ loads the \AMSmathLogo\ package
\cite{amslatex3project2019}
to do mathematics.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
There are two types of mathematics in \LaTeXLogo.
Text math is interspersed with text.
For example,
this is text math: \(a = b + c\).
Display math is not interspersed with text.
For example,
this is display math:
\begin{equation}
  a = b + c
\end{equation}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}


\section{Text Math}

Use |\(|
to start text math
and |\)|
to end text math.
Some people use |$|
to start and end text math---I don't
recommend that because \LaTeXLogo\ can give better error messages
if you use |\(|
and |\)|
\cite{meckes2010}.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}


\section{Display Math}

Use one of the below environments to start and end display math.
Some people use |$$|
to start and end displayed math
but \LaTeXLogo\ doesn't officially support |$$|
\cite{alpert2010}.


\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}


\subsection{Displayed Equations}

Do not use
|$$|
to start or end displayed math like \TeXLogo\ uses
\cite{gratzer2016}.
\todoerror{add page number to reference}

The \AMSmathLogo\ package provides a number
of additional displayed equation structures
beyond the ones provided in basic \LaTeX.
The augmented set includes
\cite{amslatex3project2019b}:

\hbox to\hsize{%
  \hss
  \begin{tabular}{@{}ll@{}}
    \toprule
    \bfseries Environment& \bfseries Used for\\
    \midrule
    \tt equation& used for single equations\\
    \tt multline& split single equations over multiple lines\\
    \tt gather& collect but do not align multiple equations\\
    \tt align& align multiple equations\\
    \tt alignat& aligns multiple equations at multiple places\\
    \tt flalign& aligns multiple equations at multiple places on full length lines\\
    \tt split& split a single equation over multiple lines\\
    \bottomrule
  \end{tabular}%
  \hss
}

All but
|split|
can be followed by
|*|
to not number equations.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsubsection{\texttt{equation} environment}

The
|equation|
environment is used for single equations.

\begin{equation}
  E = mc^2
\end{equation}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

The
|equation*|
environment does single, unnumbered equations.

\begin{equation*}
  a = b_0c + \frac12 de^2 + {\textstyle \frac12} fg^2
    + h_1 + h_2 + \cdots + h_n
    \qquad \text{for \(c \ne d\) and \(g < \infty\)}
\end{equation*}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\textcite{greene-2021-03-14}
wrote
% \begin{quotation}
  For
  \href{https://twitter.com/hashtag/PiDay?src=hashtag\_click\#PiDay}{\#PiDay},
  one of the coolest formulae for today's honoree:
  \[
    \frac 1\pi
    =
    \frac {\sqrt8} {9801}
    \sum_{n=0}^\infty
    \frac  {(4n!) (1103+26390n)}  {(n!)^4 396^{4n}}
  \]
% \end{quotation}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

The formula for Bekenstein-Hawking entropy:

\begin{equation*}
  S_\text{BH}
  =
  \frac A {4L_P^2}
  = \frac {c^3A} {4G\hbar}
\end{equation*}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

Type in the math and let \LaTeX\ worry about the spacing.
You only need to do fine tuning by hand if it looks bad.

Another
|equation*|
environment,
note the spacing before the large close parenthesis:

\begin{equation*}
  \frac ab
    = ab^{-1}
    % Parens are the wrong size.
    = (\sqrt{\frac ab})^2
    % Parens are the right size but closing paren is too close to radical.
    = \left( \sqrt\frac ab \right)^2
    % Parens are right size but a negative thin space puts closing paren on top of radical.
    = \left( \sqrt\frac ab \!\right)^2
    % Parens are right size but a thin space puts closing paren too close to radical.
    = \left( \sqrt\frac ab \,\right)^2
    % Parens are right size but a medium space puts closing paren too close to radical.
    = \left( \sqrt\frac ab \:\right)^2
    % Parens are right size and I think a thick space looks the best.
    = \left( \sqrt\frac ab \;\right)^2
\end{equation*}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{equation*}
  (\cos x)^2 + (\sin x)^2 = \cos^2 x + \sin^2 x = 1
\end{equation*}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{equation}
  x \mod 2 =
  \begin{cases}
    0& \text{if \(x\) is even}\\
    1& \text{if \(x\) is odd}\\
  \end{cases}
\end{equation}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

The first six derivatives of distance are velocity, acceleration, jerk, snap, crackle,
and pop
\cite{reid2013}.
\ix{distance//velocity//acceleration//jerk//snap//crackle//pop}

\begin{equation}
  % Every array element should be in \displaystyle (a big font).
  \AtBeginEnvironment{array}{\everymath{\displaystyle}}
  % Set space between columns to zero, use {} = ... to add a little space before the = "by hand".
  \arraycolsep = 0pt
  \text{distance derivitives} = \left\{\ %
    \begin{array}{llllllll}
      % I'm formatting the first 4 lines different from the last 3 so this will fit on one page.
      x&      {}=\text{distance}&     {}=vt\\[2pt]
      v&      {}=\text{velocity}&     {}=\frac{\di x}{\di t}\\[9pt]
      a&      {}=\text{acceleration}& {}=\frac{\di v}{\di t}& {}=\frac{\di^2x}{\di t^2}\\[9pt]
      \mit j& {}=\text{jerk}&         {}=\frac{\di a}{\di t}& {}=\frac{\di^2v}{\di t^2}&
        {}=\frac{\di^3x}{\di t^3}\\[9pt]
      s
        & {}=\text{snap}
        & {}=\frac{\di \mit j}{\di t}
        & {}=\frac{\di^2a}{\di t^2}
        & {}=\frac{\di^3v}{\di t^3}
        & {}=\frac{\di^4x}{\di t^4}\\[9pt]
      c
        & {}=\text{crackle}
        & {}=\frac{\di s}{\di t}
        & {}=\frac{\di^2\mit j}{\di t^2}
        & {}=\frac{\di^3a}{\di t^3}
        & {}=\frac{\di^4v}{\di t^4}
        & {}=\frac{\di^5x}{\di t^5}\\[9pt]
      p
        & {}=\text{pop}
        & {}=\frac{\di c}{\di t}
        & {}=\frac{\di^2s}{\di t^2}
        & {}=\frac{\di^3\mit j}{\di t^3}
        & {}=\frac{\di^4a}{\di t^4}
        & {}=\frac{\di^5v}{\di t^5}
        & {}=\frac{\di^6x}{\di t^6}
    \end{array}
  \right.
\end{equation}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsubsection{\texttt{multline} environment}

The
|multline|
environment is used
to split single equations over multiple lines.

\begin{multline}
  S = a + b + c + d + e + f + g + h + i + j\\
  + k + l + m + n + o + p\\
  + q + r + s + t + u + v + w + x + y + z
\end{multline}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{multline}
  S = a + b + c + d + e\\
  + f + g + h + i + j\\
  + k + l + m + n + o\\
  + p + q + r + s + t\\
  + u + v + w + x + y\\
  + z
\end{multline}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

% Calculate width of space before equation plus equation number.
% (All digits are the same width.)
\newdimen{\tdimen}
\settowidth{\tdimen}{\kern\multlinetaggap (L.5)}
\begin{multline}
  S = a + b + c + d + e\\
  \makebox[\textwidth]{\hfill \(+ f + g + h + i + j\)\hfill\hfill\hfill\hfill\kern\tdimen}\\
  \makebox[\textwidth]{\hfill\hfill\({} + k + l + m + n + o\)\hfill\hfill\hfill\kern\tdimen}\\
  \makebox[\textwidth]{\hfill\hfill\hfill\({} + p + q + r + s + t\)\hfill\hfill\kern\tdimen}\\
  \makebox[\textwidth]{\hfill\hfill\hfill\hfill\({} + u + v + w + x + y\)\hfill\kern\tdimen}\\
  + z
\end{multline}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsubsection{\texttt{gather} environment}

The
|gather|
environment collects but does not align multiple equations.

\begin{gather}
  a = b + c + d + e + f + g + h + i + j + k + l\\
  m = n + o + p + q + r + s + t + u + v + w + x + y + z
\end{gather}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{gather}
  a = b + c + d + e + f + g + h + i + j + k + l\notag\\
  m = n + o + p + q + r + s + t + u + v + w + x + y + z
\end{gather}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{gather*}
  \alpha = \beta + \gamma + \delta + \eta\\
  \theta = \iota + \kappa + \lambda + \mu + \nu + \rho + \tau
\end{gather*}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{gather}
  x_\text{min} + x_\text{max} \le \sum_{i=1}^n x_i\\
  x_\text{min} + x_\text{max}
    = \sum_{i=1}^n x_i - \sum_{i=2}^{n-1} x_i\quad\text{if \(x\) is sorted}\\
  x_\text{min} \le \left(\sum_{i=1}^n x_i\right) / n
\end{gather}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsubsection{\texttt{align} environment}

The
|align|
environment aligns multiple equations.

\begin{align}
  a &= b + c + d\\
  e &= f + g + h + i + j
\end{align}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{align}
  x = \frac{-b \pm \sqrt{b^2-4ac}}{2a}\notag\\
  % Put a thin space before the b^2 to improve the appearance.
  x = \frac{-b \pm \sqrt{\,b^2-4ac}}{2a}
\end{align}
\end{VerbatimOut}
\ix{align environment}
\index{\verb+\begin{align}+}
\ix{thin space}
\index{\verb+\,+}

\MyIO


\begin{VerbatimOut}{z.out}

Quadratic formula proof
\cite{khan2018}:
\ix{quadratic formula}

% The align environment requires the amsmath package.
% Use \addtolength{\jot}{6pt} to increase the space between rows in an amsmath multi-line math formula.
% That's not done here so everything will fit on one page.
\begin{align}
  ax^2 + bx + c &= 0\\
  ax^2 + bx &= -c\notag\\
  % The "\," adds a thinspace of horizontal space.
  x^2 + \frac ba\,x &= -\frac ca\notag\\
  x^2 + \frac ba\,x + \frac{b^2}{4a^2} &= \frac{b^2}{4a^2} - \frac ca\notag\\
  \left(x + \frac b{2a}\right)^2 &= \frac{b^2}{4a^2} - \frac ca\notag\\
  \left(x + \frac b{2a}\right)^2 &= \frac{b^2}{4a^2} - \frac{4ac}{4a^2}\notag\\
  \left(x + \frac b{2a}\right)^2 &= \frac{b^2-4ac}{4a^2}\notag\\
  \sqrt{\left(x + \frac b{2a}\right)^2}
    &= \sqrt{\left(\frac{b^2-4ac}{4a^2}\right)}\notag\\
  x + \frac b{2a} &= \pm \frac{\sqrt{\,b^2-4ac}}{\sqrt{4a^2}}\notag\\
  x + \frac b{2a} &= \pm \frac{\sqrt{\,b^2-4ac}}{2a}\notag\\
  x &= - \frac b{2a} \pm \frac{\sqrt{\,b^2-4ac}}{2a}\notag\\
  x &= \frac{-b \pm \sqrt{\,b^2-4ac}}{2a}
\end{align}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsubsection{\texttt{alignat} environment}
\index{\verb+\begin{aligo}+@\verb+\begin{alignat}+}
\ix{alignat environment}

The
|alignat|
environment aligns multiple equations at multiple places.
\begin{alignat}{2}
  a &= b& \qquad\qquad& \text{set \(a\)}\\
  c &= d& &             \text{you guessed it, set \(c\)}\notag\\
  g &= h& &             \text{and finally, set \(g\)}
\end{alignat}
\index{\verb+\begin{aligo}+@\verb+\begin{alignat}+}
\ix{alignat environment}

I like to align input columns on the input if possible
and will sometimes use windows over~250 characters wide to do so.
If that won't work I sometimes do,
for example,
\begin{alignat}{2}
  a
    &= b
    & \qquad\qquad
    & \text{set \(a\)}\\
  c
    &= d
    &
    &\text{you guessed it, set \(c\)}\notag\\
  g
    &= h
    &
    &\text{and finally, set \(g\)}
\end{alignat}
\index{\verb+\begin{aligo}+@\verb+\begin{alignat}+}
\ix{alignat environment}

Do whatever works best for you.

\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

Quadratic formula proof
\cite{khan2018}:

% Make changes to \jot be local to the group that starts on the next line.
{
  % Increase distance between lines by 6pt.
  \addtolength{\jot}{6pt}
  \begin{alignat}{2}
    ax^2 + bx + c
      &= 0
      &
      &\text{subtract \(c\)}\\
    ax^2 + bx
      &= -c
      &
      &\text{divide by \(a\)}\notag\\
    % The "\," adds a thinspace of horizontal space.
    x^2 + \frac ba\,x
      &= -\frac ca
      &
      &\text{add \(\displaystyle\frac{b^2}{4a^2}\)}\notag\\
    x^2+\frac ba\,x+\frac{b^2}{4a^2}
      &= \frac{b^2}{4a^2}-\frac ca
      &
      &\text{factor left hand side}\notag\\
    \left(x+\frac b{2a}\right)^2
      &= \frac{b^2}{4a^2}-\frac ca
      &
      &\text{multiply right-most term by \(\displaystyle\frac{4a}{4a}\)}\notag\\
    \left(x + \frac b{2a}\right)^2
      &= \frac{b^2}{4a^2}-\frac{4ac}{4a^2}
      &
      &\text{use common denominator}\notag\\
    \left(x + \frac b{2a}\right)^2
      &= \frac{b^2-4ac}{4a^2}
      &
      &\text{take square root of each side}\notag\\
    \sqrt{\left(x + \frac b{2a}\right)^2}
      &= \sqrt{\left(\frac{b^2-4ac}{4a^2}\right)}
      &
      &\text{compute square root of each side}\notag\\
    x + \frac b{2a}
      &= \pm \frac{\sqrt{\,b^2-4ac}}{\sqrt{4a^2}}
      &
      &\text{simplify right hand denominator}\notag\\
    x + \frac b{2a}
      &= \pm \frac{\sqrt{\,b^2-4ac}}{2a}
      &
      &\text{subtract \(\displaystyle\frac b{2a}\) from each side}\notag\\
    x
      &= -\frac b{2a} \pm \frac{\sqrt{\,b^2-4ac}}{2a}
      &\qquad
      &\text{use common denominator}\notag\\
    x
      &= \frac{-b \pm \sqrt{\,b^2-4ac}}{2a}
  \end{alignat}
}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\index{\verb+\begin{flalign}+}
\todoindex{Verb+Begin-Ocurly-flalign-Ccurly+}
\ix{falign environment}
\subsubsection{\texttt{flalign} environment}

The
|flalign|
environment aligns multiple equations at multiple places
on full length lines.

\begin{flalign}
  a &= b&   &   & u &= v\\
  c &= d& m &= n& w &= x\notag\\
  g &= h&   &   & y &= z
\end{flalign}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\index{\verb+\begin{split}+}
\todoindex{Verb+Begin-Ocurly-split-Ccurly+}
\ix{split environment}
\subsubsection{\texttt{split} environment}

The
|split|
environment ???.
\index{\verb+\begin{split}+}
\todoindex{Verb+Begin-Ocurly-split-Ccurly+}
\ix{split environment}


\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}


\newpage
\section{Use the Following in Text or Display Math}

The following constructs can be used in text or display math.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{Breaking Lines}

This information is based on information from ISO 80000-2
\cite[page 2]{iso80000-2}:
\begin{quote}
  If an expression or equation must be split into two or more lines,
  place the line breaks immediately before one of the symbols
  \(=\),
  \(+\),
  \(-\),
  \(\times\),
  \(/\),
  \(\pm\),
  \(\mp\),
  etc.
\end{quote}

Examples:

The alternating sum of the first 20 prime numbers is
\(2 - 3 + 5 - 7 + 11 - 13 + 17 - 19\\+ 23 - 29 + 31 - 37 + 41 - 43 + 47 -53 + 59 - 61 + 67 - 71\).
\begin{align}
  s = {} & 2 - 3 + 5 - 7 + 11 - 13 + 17 - 19 + 23 - 29\nonumber\\
         & + 31 - 37 + 41 - 43 + 47 -53 + 59 - 61 + 67 - 71\nonumber
\end{align}

\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{Constants, etc., should be in an upright font}

This information is based on information
in ISO 80000-2
\cite[page 1]{iso80000-2}:
\begin{itemize}
  \item
    The constants \(\mit e\),~\(\mit i\),~\(\mit j\), and~\(\itpi\)
    should be typeset in an upright font as \(e\),~\(i\),~\(j\) and~\(\pi\).\\
    Example: \(\displaystyle e^{i\pi} + 1 = 0\).
  \item
    The ordinary derivative operator \(d\)
    should be typeset in an upright font as `\(\mathrm{d}\)'.\\
    Example: \(\displaystyle \int 2x\di x = x^2 + C\).
  \item
    The partial derivative operator \(\partial\)
    should be typeset in an upright font as \(\pa\).
    Example:
    \(
      \displaystyle
      \frac {\pa f} {\pa x}
      =
      f_x
      =
      \lim_{h\to 0}
      \frac {f(x + h,y) - f(x,y)} {h}
      =
      \lim\nolimits_{h\to 0}
      \frac {f(x + h,y) - f(x,y)} {h}
    \).
\end{itemize}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
\newpage
The |thesis.tex| file sets up the first capability above with
\begin{verbatim}
% Follow ISO 80000-2:2019
%     o   put e, i, j, and pi in upright font automatically
%     o   use, for example, "\di x" to get "\,mathrm{d}\/x"
\usepackage{pa-mismath}
  % Put e, i, j, and pi in upright font automatically.
  % Comment the corresponding line to not put the symbol in an upright font.
  \enumber
  \inumber
  \jnumber
  \pinumber
  % With the four lines above not commented out, to typeset math italic e,
  % i, j, and pi use
  %     \mathit e
  %     \mathit i
  %     \mathit j
  %     \itpi
\end{verbatim}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
\subsection{English Words}

English words in math should be in a roman font like this:\\
Let the maximum value of \(a\) be \(a_\text{max}\).\\
\(a_\text{max} \ge a_\text{min}\) should always be true.\\
The temperature in the attic is \(t_\text{attic}\).
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{Functions}

Standard functions should be in a roman font.
Like this: \(\cos\theta\).
Here is a list of standard function commands:\\

% The "@{\hspace*{\parindent}}" indents the table
% the same amount as a paragraph.
\begin{tabular}{@{\hspace*{\parindent}}llll@{}}
  \verb+\arccos+& \verb+\csc+& \verb+\ker+&    \verb+\min+\\
  \verb+\arcsin+& \verb+\deg+& \verb+\lg+&     \verb+\Pr+\\
  \verb+\arctan+& \verb+\det+& \verb+\lim+&    \verb+\sec+\\
  \verb+\arg+&    \verb+\dim+& \verb+\liminf+& \verb+\sin+\\
  \verb+\cos+&    \verb+\exp+& \verb+\limsup+& \verb+\sinh+\\
  \verb+\cosh+&   \verb+\gcd+& \verb+\ln+&     \verb+\sup+\\
  \verb+\cot+&    \verb+\hom+& \verb+\log+&    \verb+\tan+\\
  \verb+\coth+&   \verb+\inf+& \verb+\max+&    \verb+\tanh+\\
\end{tabular}
\ix
{%
  arccos//arcsin//arctan//arg//cos//cosh//cot//coth%
  //csc//deg//det//dim//exp//gcd//hom//inf%
  //ker//lg//lim//liminf//limsup//ln//log//max%
  //min//Pr//sec//sin//sinh//sup//tan//tanh%
}
\index{\verb+\arccos+} \index{\verb+\arcsin+} \index{\verb+\arctan+} \index{\verb+\arg+}
\index{\verb+\cos+} \index{\verb+\cosh+} \index{\verb+\cot+} \index{\verb+\coth+}
\index{\verb+\csc+} \index{\verb+\deg+} \index{\verb+\det+} \index{\verb+\dim+}
\index{\verb+\exp+} \index{\verb+\gcd+} \index{\verb+\hom+} \index{\verb+\inf+}
\index{\verb+\ker+} \index{\verb+\lg+} \index{\verb+\lim+} \index{\verb+\liminf+}
\index{\verb+\limsup+} \index{\verb+\ln+} \index{\verb+\log+} \index{\verb+\max+}
\index{\verb+\min+} \index{\verb+\Pr+} \index{\verb+\sec+} \index{\verb+\sin+}
\index{\verb+\sinh+} \index{\verb+\sup+} \index{\verb+\tan+} \index{\verb+\tanh+}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{Matrices}

From ISO 80000-2
\cite[page 18]{iso80000-2}:
\begin{quotation}
  Matrices are usually written with boldface italic capital letters
  and their elements with italic lower case letters,
  but other typefaces may be used.
  \todoerror{Double check this quote.}
\end{quotation}

Example:
Let \(\bm{M}\) be a \(3 \times 3\) matrix:
\begin{equation*}
  \bm{M}
  =
  \left(
    \begin{array}{ccc}
      m_{1,1}& m_{1,2}& m_{1,3}\\
      m_{2,1}& m_{2,2}& m_{2,3}\\
      m_{3,1}& m_{3,2}& m_{3,3}\\
    \end{array}
  \right)
  =
  \left(
      % If your thesis.tex is set up to assume, for example, 'e' is a constant
      % and typeset in an upright font, use '\mit e' to typeset 'e' in a math
      % italic font.
    \begin{array}{ccc}
      a& b& c\\
      d& \mit e& f\\
      g& h& \mit i\\
    \end{array}
  \right)
\end{equation*}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{Sets}

% Make \newcommand local to { ... }.
{
  % \St is short for my set.
  \newcommand{\Se}[1]{\ensuremath{\mathbf #1}}
  % \St is short for suchthat.
  \newcommand{\St}{\mid}
  \noindent
  Use \(\mathbb{N}\) for the natural numbers.
  \index{natural numbers}\\
  Use \(\mathbb{R}\) for the real numbers.
  \index{real numbers}\\
  Use \(\mathbb{Z}\) for the integers.
  \index{integers}\\
  The Cartesian product\index{\verb+\times+}\index{Cartesian product}
  of \Se A and \Se B is
  \(\Se A \times \Se B = \{(a,b) \St a \in \Se A \text{ and } b \in \Se B\}\).\\
  The intersection\index{\verb+\cap+}\index{intersection}
  of \Se A and \Se B is
  \(\Se A \cap \Se B = \{ x \St x \in \Se A \text{ and } x \in \Se B\}\).\\
  The union\index{\verb+\cup+}\index{union}
  of \Se A and \Se B is
  \(\Se A \cup \Se B = \{ x \St x \in \Se A \text{ and } x \in \Se B\}\).
}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}


\section{Theorem-like environments}

The |ntheorem| package\index{ntheorem package}
is used instead of |amsthm|\index{amsthm package}
so the counter
for a theorem-like construct
can be overridden by the user.
See
\cite[pages 4--5]{may2011}
and below
for how to do this.
\end{VerbatimOut}

\MyIO


% This list was made using data in
%     https://ctan.math.utah.edu/ctan/tex-archive/macros/latex/required/amscls/doc/amsthdoc.pdf
% which was used to make a list of definitions in PurdueThesis.cls
%     acknowledgment
%     assertion
%     assumption
%     axiom
%     case
%     claim
%     conclusion
%     condition
%     conjecture
%     corollary
%     criterion
%     definition
%     example
%     exercise
%     hypothesis
%     lemma
%     notation
%     note
%     observation (was defined in a earlier version of PurdueThesis)
%     problem
%     proof (is defined by ntheorem package)
%     property
%     proposition
%     question
%     remark
%     summary
%     theorem


\begin{VerbatimOut}{z.out}

By default all theorem-like constructs:\\[6pt]
\begin{tabular}{@{\hspace*{2\parindent}}llllll@{}}
acknowledgment& assertion&  assumption& axiom&      case&        claim\\
conclusion&     condition&  conjecture& corollary&  criterion&   definition\\
example&        exercise&   hypothesis& lemma&      notation&    note\\
observation&    problem&    proof&      property&   proposition& question\\
remark&         summary&    theorem\\
\end{tabular}
\mbox{}\\[6pt]
use the same counter.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

From PurdueThesis.cls:
\begin{verbatim}
    \usepackage[amsthm]{ntheorem}
      % From example 31 of https://math.mit.edu/~poonen/papers/writing.pdf
      %     Use a single numbering system for all theorems, lemmas, etc.,
      %     instead of having both a Theorem 1.1 and a Lemma 1.1 in the
      %     same paper. This makes statements easier to find[...]
      % For example,
      %     \newtheorem{lemma}[theorem]{Lemma}
      % makes lemma use the theorem counter.
      \theoremstyle{plain}
      \newtheorem{theorem}{Theorem}[section]
      \newtheorem{lemma}[theorem]{Lemma}
      [28 more lines]
\end{verbatim}
To make,
for example,
lemma have its own counter put
\begin{verbatim}
    \renewtheorem{lemma}{Lemma}[section]
\end{verbatim}
in your thesis.tex file right after the |\begin{document}| statement.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{acknowledgment}
  \MyRepeat{This is a sentence.  }{5}
\end{acknowledgment}
\index{\verb+\begin{acknowledgment}+}
\index{acknowledgment environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{assertion}
  \MyRepeat{This is a sentence.  }{5}
\end{assertion}
\index{\verb+\begin{assertion}+}
\index{assertion environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{assumption}
  \MyRepeat{This is a sentence.  }{5}
\end{assumption}
\index{\verb+\begin{assumption}+}
\index{assumption environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{axiom}
  \MyRepeat{This is a sentence.  }{5}
\end{axiom}
\index{\verb+\begin{axiom}+}
\index{axiom environment}
\end{VerbatimOut}

\MyIO


% \begin{VerbatimOut}{z.out}
%
% \begin{case}
%   \MyRepeat{This is a sentence.  }
% \end{case}
% \index{\verb+\begin{case}+}
% \index{case environment}
% \end{VerbatimOut}
%
% \MyIO


\begin{VerbatimOut}{z.out}

\begin{claim}
  \MyRepeat{This is a sentence.  }{5}
\end{claim}
\index{\verb+\begin{claim}+}
\index{claim}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{conclusion}
  \MyRepeat{This is a sentence.  }{5}
\end{conclusion}
\index{\verb+\begin{conclusion}+}
\index{conclusion environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{condition}
  \MyRepeat{This is a sentence.  }{5}
\end{condition}
\index{\verb+\begin{condition}+}
\index{condition environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{conjecture}
  \MyRepeat{This is a sentence.  }{5}
\end{conjecture}
\index{\verb+\begin{conjecture}+}
\index{conjecture environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{corollary}
  \MyRepeat{This is a sentence.  }{5}
\end{corollary}
\index{\verb+\begin{corollary}+}
\index{corollary environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{criterion}
  \MyRepeat{This is a sentence.  }{5}
\end{criterion}
\index{\verb+\begin{criterion}+}
\index{criterion environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{definition}
  \MyRepeat{This is a sentence.  }{5}
\end{definition}
\index{\verb+\begin{definition}+}
\index{definition environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{example}
  \MyRepeat{This is a sentence.  }{5}
\end{example}
\index{\verb+\begin{example}+}
\index{example environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{exercise}
  \MyRepeat{This is a sentence.  }{5}
\end{exercise}
\index{\verb+\begin{exercise}+}
\index{exercise environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{hypothesis}
  \MyRepeat{This is a sentence.  }{5}
\end{hypothesis}
\index{\verb+\begin{hypothesis}+}
\index{hypothesis environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{lemma}
  \MyRepeat{This is a sentence.  }{5}
\end{lemma}
\index{\verb+\begin{lemma}+}
\index{lemma environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{notation}
  \MyRepeat{This is a sentence.  }{5}
\end{notation}
\index{\verb+\begin{notation}+}
\index{notation environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{note}
  \MyRepeat{This is a sentence.  }{5}
\end{note}
\index{\verb+\begin{note}+}
\index{note environment}
\end{VerbatimOut}

\MyIO


% \begin{VerbatimOut}{z.out}
%
% \begin{observation}
%   \MyRepeat{This is an example observation.  }{5}
% \end{observation}
% \index{\verb+\begin{observation}+}
% \index{observation environment}
% \end{VerbatimOut}
%
% \MyIO


\begin{VerbatimOut}{z.out}

\begin{problem}
  \MyRepeat{This is a sentence.  }{5}
\end{problem}
\index{\verb+\begin{problem}+}
\index{problem environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{proof}
  \MyRepeat{This is an example proof.  }{5}
\end{proof}
\index{\verb+\begin{proof}+}
\index{proof environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{property}
  \MyRepeat{This is a sentence.  }{5}
\end{property}
\index{\verb+\begin{property}+}
\index{property environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{proposition}
  \MyRepeat{This is an example proposition.  }{5}
\end{proposition}
\index{\verb+\begin{proposition}+}
\index{proposition environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{question}
  \MyRepeat{This is a sentence.  }{5}
\end{question}
\index{\verb+\begin{question}+}
\index{question environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{remark}
  \MyRepeat{This is a sentence.  }{5}
\end{remark}
\index{\verb+\begin{remark}+}
\index{remark environment}
\end{VerbatimOut}

\MyIO


% There is already a \rule command.
% \begin{VerbatimOut}{z.out}
%
% \begin{rule}
%   This is an example rule.
%   This is an example rule.
%   This is an example rule.
%   This is an example rule.
%   This is an example rule.
% \end{rule}
% \index{\verb+\begin{rule}+}
% \index{rule environment}
% \end{VerbatimOut}
%
% \MyIO


% \begin{VerbatimOut}{z.out}
%
% \begin{solution}
%   \MyRepeat{This is an example solution.  }{5}
% \end{solution}
% \index{\verb+\begin{solution}+}
% \index{solution environment}
% \end{VerbatimOut}
%
% \MyIO


\begin{VerbatimOut}{z.out}

\begin{summary}
  \MyRepeat{This is a sentence.  }{5}
\end{summary}
\index{\verb+\begin{summary}+}
\index{summary environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{theorem}
  \MyRepeat{This is an example theorem.  }{5}
\end{theorem}
\index{\verb+\begin{theorem}+}
\index{theorem environment}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}


\section{Examples}

\subsection{Bayes' Theorem}
\ix{Bayes' Theorem}
\ix{Bayes, Thomas}

Bayes' Theorem
\cite{bayes}
is
{
  \UndefineShortVerb{\|}
  \begin{equation}
    \text{P}(\text A|\text B)
    % The "\," puts a thin horizontal space there, 1/6 of an "em".
    % An "em" is roughly the width of a lowercase "m".
    = \frac{\text P(\text B|\text A)\,\text P(\text A)}{\text P(\text B)}
  \end{equation}
}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{Euler's identity}
\ix{Euler's identity}
\ix{Euler, Leonhard}

Euler's identity
\cite{eulers-identity}
is
\begin{equation}
  e^{i\pi} + 1 = 0.
\end{equation}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{Fourier transform}
\ix{Fourier Transform}

ISO 80000-2
\cite[page 25]{iso80000-2}
recommends using
\(\Fourier\)
nfor the Fourier transform.
The Fourier transform of \(f\) is
\(
  \displaystyle
  (\Fourier f)(\omega)
  = \Fourier (\omega)
  = \int_{-\infty}^\infty e^{i\omega t} f(t) \di t
\).
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{Laplace transform}
\ix{Laplace Transform}

ISO 80000-2
\cite[page 25]{iso80000-2}
recommends using
\(\Laplace\)
for the Laplace transform.
The Laplace transform of \(s\) is
\(
  \displaystyle
  (\Laplace f)(s)
  = \Laplace(s)
  = \int_0^\infty e^{-st} f(t) \di t
\).
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{Nicomachus's theorem}
\ix{Nicomachus's theorem}
\ix{Nicomachus of Gerasa}
Nicomachus's theorem
\cite{wikipedia-nicomachus}
states that
the sum of the first~\(n\) cubes is the square of the~\(n\)th triangular number.
That is,
\begin{equation}
  1^3 + 2^3 + 3^3 + \cdots + n^3 = (1 + 2 + 3 + \cdots + n)^2.
\end{equation}
The same equation may be written more compactly using the mathematical notation for summation:
\begin{equation*}
  \sum_{k=1}^n k^3 = \left(\sum_{k=1}^n k\right)^2.
\end{equation*}
Also see the diagram on that web page.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{Prime Number Theorem}
\ix{Prime Number Theorem}

\textcite{li2013}
\ix{Li, Henry}
suggested using a functional equation
from the Prime Number Theorem proof
as an example:
\begin{equation}
  \int_1^x
    \sum_{p\le u}
    \left\lfloor\frac{\log u}{\log p}\right\rfloor
    \log p
    \di u
    =
    \frac1{2\pi i}
    \int_{c-i\infty}^{c+i\infty}
    \frac{x^{s+1}}{s(s+1)}
    \left(-\frac{\zeta'(s)}{\zeta(s)}\right)
    \di s
\end{equation}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{Quantum Mechanics}
\ix{Quantum Mechanics}

\textcite{greene-2021-04-04}
wrote
\ix{Greene, Brian Randolph}
\begin{quotation}
  Quantum Mechanics in a nutshell:
  A particle goes from here to there
  by sampling every possible trajectory from here to there.

  \[
    \langle x_f,t_f \mid x,t_{\mathit i} \rangle
    =
    \sum_{\text p \in \text{paths}} e^{\mathit iS(\text p) \si{\planckbar}}
  \]
\end{quotation}
\end{VerbatimOut}

\MyIO


%  https://tex.stackexchange.com/questions/96568/how-can-i-align-multiple-cases-environment-simultaneously
\begin{VerbatimOut}{z.out}

\subsection{Question in String Theory / Mass of States / Number Operator}

\textcite{yourlazyphysicist2017}
wrote
``I have the following definition of the space-time coordinates'':
{
  % The following five definitions are local to inside the { ... }.
  \newcommand{\fpt}{{4\pi T}}
  \newcommand{\oh}{\frac12}
  \newcommand{\snnz}{\sum_{n\ne0}}
  \newcommand{\tms}{\tau - \sigma}
  \newcommand{\tps}{\tau + \sigma}
  \begin{align}
    \text{closed string: }&
      \begin{cases}
        \displaystyle
        X^\mu_R
          = \oh x^\mu
          + \frac1\fpt (\tms) p^\mu
          + \frac i{\sqrt\fpt} \snnz \frac1n \alpha^\mu_n e^{-in(\tms)},\\
        \displaystyle
        X^\mu_L
          = \oh x^\mu
          + \frac1\fpt (\tps) p^\mu
          + \frac i{\sqrt\fpt} \snnz \frac1n \tilde\alpha^\mu_n e^{-in(\tps)}.
      \end{cases}\\[6pt]
    \text{open string: }&
      \begin{cases}
        \displaystyle
        X^\mu_N
          = x^\mu
          + \frac1{\pi T}p^\mu\tau
          + \frac i{\sqrt{\pi T}} \snnz \frac1n \alpha^\mu_n e^{-in\tau} \cos(n\sigma),\\
        \displaystyle
        X^\mu_D
          = x^\mu
          + \frac i{\sqrt{\pi T}} \snnz \frac1n \alpha^\mu_n e^{-in\tau} \sin(n\sigma).
      \end{cases}
  \end{align}
}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{Willans' Formula}

\citetitle{rowland2022}
\cite{rowland2022}
\ix{Willans, C. P.}
\ix{Rowland, Eric Samuel}
is a good video about Willans' Formula by Eric Rowland:

\begin{equation}
  % Typeset i and j in a math italic font for this equation only.
  \MathIt{i}
  \MathIt{j}
  \text{\(n\)th prime}
  =
  1
  +
  \sum_{i = 1}^{2^n}
  \left\lfloor
    \left(
      \frac
        n
        {
          \displaystyle  % so \sum limits are above and below and to make denominator bigger
          \sum_{j=1}^i
          \left\lfloor
            \left(
              % use \, for a tiny bit of horizontal space
              \cos \pi \, \frac {(j-1)! + 1} j
            \right)^2
          \right\rfloor
        }
    \right)^{1/n}
  \right\rfloor
\end{equation}
\end{VerbatimOut}

\MyIO




% https://www.google.com/url?sa=i&rct=j&q=&esrc=s&source=images&cd=&cad=rja&uact=8&ved=0ahUKEwiSzf370-jmAhXIGs0KHRHyAZQQMwiCASgNMA0&url=https%3A%2F%2Fwww.chegg.com%2Fhomework-help%2Fquestions-and-answers%2Fequations-displacement-atoms-along-linear-chain-d2u-u-m-mass-atoms-c-force-constant-neares-q26052186&psig=AOvVaw1eYq-Q0El0Tbjgbp_Lu2Vv&ust=1578183004388936&ictx=3&uact=3

% M\frac{d^2\mu_n}{dt^2} = C(u_{n_1} - 2u_n + u_{n-1}).

% a^{b} same as a^b     c^{de} f^{g^h} ij^{kl}^{mn}

% superscripts
% subscripts

% operators

%\sum
%\prod

%\alpha
%\beta
%\gamma
%\delta
%\epsilor
%\varepsilon
%\zero
%\eta
%\theta
%\vartheta
%\iota
%\kappa
%\lambda
%\mu
%\nu\xi
%\varrho
%\sigma
%\varsigma
%\tau
%\upsilan
%\pha
%\varphi
%\chi
%\psi
%\omega

%\Gamma
%\Delta
%\Theta
%\Lambda
%\Xi
%\Pi
%\Sigmo
%\Upsilan
%\Phi
%\Psi
%\Omega

%mixed greek and text

%x_min, x_max

%\ldots

%\to

%1 + \frac14 + \frac19 + \cdots = \frac\pi6

%fractions

% frac{\ln x}{\ln\alpha} = log_\alpha x

% \sum_{i=1}^n = 1 + 2 + \cdots + n = \frac{n(n+1)}{2}


% xxxx     \end{verbatim}
% xxxx % Requires \usepackage{amsmath}; use align* for no equation number.
% xxxx \begin{align}
% xxxx   a = {}& b + c\\
% xxxx   x = {}& y + z
% xxxx \end{align}
% xxxx     \vskip\baselineskip
% xxxx     \hrule
% xxxx     \vskip0.5\baselineskip
% xxxx     \filbreak
% xxxx
% xxxx     \begin{verbatim}
% xxxx \[
% xxxx   Z =
% xxxx     \left(
% xxxx       \begin{array}{cc}
% xxxx         a& b\\
% xxxx         c& d
% xxxx       \end{array}
% xxxx     \right)
% xxxx \]
% xxxx     \end{verbatim}
% xxxx \[
% xxxx   Z =
% xxxx     \left(
% xxxx       \begin{array}{cc}
% xxxx         a& b\\
% xxxx         c& d
% xxxx       \end{array}
% xxxx     \right)
% xxxx \]
% xxxx     \vskip\baselineskip
% xxxx     \hrule
% xxxx     \vskip0.5\baselineskip
% xxxx     \filbreak
% xxxx
% xxxx     \begin{verbatim}
% xxxx \begin{equation}
% xxxx   \begin{split}
% xxxx     a = {}& b + c\\
% xxxx       & {} + d + e
% xxxx   \end{split}
% xxxx \end{equation}
% xxxx     \end{verbatim}
% xxxx \begin{equation}
% xxxx   \begin{split}
% xxxx     a = {}& b + c\\
% xxxx       & {} + d + e
% xxxx     \end{split}
% xxxx \end{equation}
% xxxx     \vskip\baselineskip
% xxxx     \hrule
% xxxx     \vskip0.5\baselineskip
% xxxx     \filbreak
% xxxx
% xxxx     \begin{verbatim}
% xxxx \[
% xxxx   (\cos x)^2 + (\sin x)^2 = 1
% xxxx \]
% xxxx     \end{verbatim}
% xxxx \[
% xxxx   (\cos x)^2 + (\sin x)^2 = 1
% xxxx \]
% xxxx     \vskip\baselineskip
% xxxx     \hrule
% xxxx     \vskip0.5\baselineskip
% xxxx     \filbreak
% xxxx
% xxxx     \begin{verbatim}
% xxxx If $X = \cos x$ and $Y = \sin x$ then $X^2 + Y^2 = 1$.
% xxxx     \end{verbatim}
% xxxx If $X = \cos x$ and $Y = \sin x$ then $X^2 + Y^2 = 1$.
% xxxx     \vskip\baselineskip
% xxxx     \hrule
% xxxx     \vskip0.5\baselineskip
% xxxx     \filbreak
% xxxx
% xxxx


==> ap-publications.tex <==
\ProvidesFile{ap-publications.tex}[2023-06-06 publications appendix]

\ZZnonchapter{odd}{PUBLICATION(S)}{y}{0pt}
\ix{publication environment//publications environment}
\index{\verb+\begin{publicationa}+@\verb+\begin{publication}+}
\index{\verb+\begin{publications}+}
    
The following is based on information in
\cite{template1,template2,template3}.

\renewcommand{\I}{\hspace*{2\ZZparindent}$\bullet$\hspace*{1.5em}}

In a publication or publications section you can\\
  \I list a single publication\index{publication environment}\\
  \I include a single publication\\
  \I list multiple publications\index{publications environment}\\
  \I include multiple publications\\
Use\newline
\hspace*{0.5in}\verb+\begin{publication}+\ldots\verb+\end{publication}+\newline
or\newline
\hspace*{0.5in}\verb+\begin{publications}+\ldots\verb+\end{publications}+\newline
to skip to the next page and put the appropriate heading on the
top of the page.

\vspace*{1.5\baselineskip}

\section*{To Include a Single Publication}

\begin{verbatim}
  \begin{publication}
    ...put a single publication here...
    ...IMPROVE THIS LATER to show how to do that...
  \end{publication}
\end{verbatim}


\section*{To List Publications}

Add\\
\I |keywords = {publication},|\\
to all
|all-biblatex.bib|
entries
that should be in the publications list.

\printbibliography
[
  keywords = {publication},
]



==> ch-mappo.tex <==
\ProvidesFile{ch-mappo.tex}[2026-04-06 MaPPO chapter]

\chapter{Preference Alignment with Prior Knowledge}
\label{ch:mappo}

\begingroup

\UndefineShortVerb{\|}

\graphicspath{{papers/mappo/}{papers/mappo/figures/}}

\makeatletter
\edef\ZZOldInputPath{\input@path}
\def\input@path{{papers/mappo/}{papers/mappo/appendix/}\ZZOldInputPath}
\makeatother

\providecommand{\citep}[1]{\cite{#1}}
\providecommand{\citet}[1]{\cite{#1}}

\definecolor{ForestGreen}{rgb}{0.13, 0.55, 0.13}
\definecolor{Apricot}{rgb}{0.98, 0.81, 0.69}


\input{papers/mappo/mappo_body_thesis.tex}

\DefineShortVerb{\|}

\endgroup

==> gr-r.tex <==
% Created by tikzDevice version 0.6.2-92-0ad2792 on 2021-11-24 17:04:02
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor[named]{fillColor}{rgb}{1.00,1.00,1.00}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (361.35,361.35);
\begin{scope}
\path[clip] ( 49.20, 61.20) rectangle (336.15,312.15);
\definecolor[named]{drawColor}{rgb}{0.00,0.00,0.00}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 59.83, 70.49) --
	( 62.48, 70.52) --
	( 65.14, 70.59) --
	( 67.80, 70.70) --
	( 70.46, 70.87) --
	( 73.11, 71.08) --
	( 75.77, 71.33) --
	( 78.43, 71.63) --
	( 81.08, 71.98) --
	( 83.74, 72.38) --
	( 86.40, 72.82) --
	( 89.05, 73.31) --
	( 91.71, 73.84) --
	( 94.37, 74.42) --
	( 97.03, 75.05) --
	( 99.68, 75.72) --
	(102.34, 76.44) --
	(105.00, 77.21) --
	(107.65, 78.02) --
	(110.31, 78.88) --
	(112.97, 79.79) --
	(115.62, 80.74) --
	(118.28, 81.74) --
	(120.94, 82.79) --
	(123.59, 83.88) --
	(126.25, 85.02) --
	(128.91, 86.20) --
	(131.57, 87.43) --
	(134.22, 88.71) --
	(136.88, 90.04) --
	(139.54, 91.41) --
	(142.19, 92.82) --
	(144.85, 94.29) --
	(147.51, 95.80) --
	(150.16, 97.36) --
	(152.82, 98.96) --
	(155.48,100.61) --
	(158.13,102.30) --
	(160.79,104.05) --
	(163.45,105.84) --
	(166.11,107.67) --
	(168.76,109.55) --
	(171.42,111.48) --
	(174.08,113.46) --
	(176.73,115.48) --
	(179.39,117.55) --
	(182.05,119.66) --
	(184.70,121.82) --
	(187.36,124.03) --
	(190.02,126.28) --
	(192.68,128.58) --
	(195.33,130.93) --
	(197.99,133.32) --
	(200.65,135.76) --
	(203.30,138.25) --
	(205.96,140.78) --
	(208.62,143.36) --
	(211.27,145.99) --
	(213.93,148.66) --
	(216.59,151.38) --
	(219.24,154.14) --
	(221.90,156.96) --
	(224.56,159.81) --
	(227.22,162.72) --
	(229.87,165.67) --
	(232.53,168.67) --
	(235.19,171.71) --
	(237.84,174.80) --
	(240.50,177.94) --
	(243.16,181.12) --
	(245.81,184.35) --
	(248.47,187.63) --
	(251.13,190.95) --
	(253.78,194.32) --
	(256.44,197.74) --
	(259.10,201.20) --
	(261.76,204.71) --
	(264.41,208.26) --
	(267.07,211.86) --
	(269.73,215.51) --
	(272.38,219.21) --
	(275.04,222.95) --
	(277.70,226.73) --
	(280.35,230.57) --
	(283.01,234.45) --
	(285.67,238.38) --
	(288.32,242.35) --
	(290.98,246.37) --
	(293.64,250.43) --
	(296.30,254.55) --
	(298.95,258.71) --
	(301.61,262.91) --
	(304.27,267.16) --
	(306.92,271.46) --
	(309.58,275.81) --
	(312.24,280.20) --
	(314.89,284.64) --
	(317.55,289.12) --
	(320.21,293.65) --
	(322.87,298.23) --
	(325.52,302.86);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (361.35,361.35);
\definecolor[named]{drawColor}{rgb}{0.00,0.00,0.00}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 59.83, 61.20) -- (325.52, 61.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 59.83, 61.20) -- ( 59.83, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (112.97, 61.20) -- (112.97, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (166.11, 61.20) -- (166.11, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (219.24, 61.20) -- (219.24, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (272.38, 61.20) -- (272.38, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (325.52, 61.20) -- (325.52, 55.20);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 59.83, 39.60) {0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (112.97, 39.60) {2};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (166.11, 39.60) {4};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (219.24, 39.60) {6};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (272.38, 39.60) {8};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (325.52, 39.60) {10};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 70.49) -- ( 49.20,302.86);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 70.49) -- ( 43.20, 70.49);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,116.97) -- ( 43.20,116.97);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,163.44) -- ( 43.20,163.44);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,209.91) -- ( 43.20,209.91);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,256.38) -- ( 43.20,256.38);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,302.86) -- ( 43.20,302.86);

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80, 70.49) {0};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,116.97) {20};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,163.44) {40};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,209.91) {60};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,256.38) {80};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,302.86) {100};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 61.20) --
	(336.15, 61.20) --
	(336.15,312.15) --
	( 49.20,312.15) --
	( 49.20, 61.20);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (361.35,361.35);
\definecolor[named]{drawColor}{rgb}{0.00,0.00,0.00}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (192.68, 15.60) {$x$};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 10.80,186.67) {$y$};
\end{scope}
\end{tikzpicture}


==> latexmkrc <==
#
#  revised  latexmkrc  2024-10-16  Mark Senn  http://engineering.purdue.edu/~mark
#  created  latexmkrc  2024-10-10  Mark Senn  http://engineering.purdue.edu/~mark
#

# This file is only used by Overleaf.
# Overleaf is used to run the TeX typesetting system on the web.?.

# A latekmkrc file can be used to augment what
# the latexmk program does on Overleaf (run LaTeX
# on the web).  See
#   https://www.overleaf.com/learn/latex/Articles/How_to_use_latexmkrc_with_Overleaf

# So \"o will work in text and {\"o} will work in biblatex bibliographies.
# Without this the accented character is not printed in the bibliography.
$biber = 'biber --output-safechars';

# Set the default timezone to Indianapolis, Indiana.
# That's the same timezone as West Lafayette, Indiana---where
# Purdue's main campus is located.
# See
#   https://www.overleaf.com/learn/latex/Articles/How_to_use_latexmkrc_with_Overleaf
# for more information.
$ENV{'TZ'} = 'America/Indiana/Indianapolis';


==> papers/contextual_integrity/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

==> papers/contextual_integrity/preamble.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
% \usepackage{xcolor}         % colors
\usepackage{pgfplotstable}

\pgfplotsset{compat=1.16}

%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
%!!!!!!                            !!!!!
%!!!!!!        IMPORTANT           !!!!!
%!!!!!!                            !!!!!
% Uncomment the next line for final version
\usepackage[disable]{todonotes}      % Disable any comments left in the document
%\usepackage{todonotes}      % Add todonotes package

\usepackage{xpatch}

\usepackage{xpatch}
\makeatletter
\xapptocmd{\NAT@bibsetnum}{\setlength{\leftmargin}{0pt}\setlength{\itemindent}{\labelwidth}\addtolength{\itemindent}{\labelsep}}{}{}
\makeatother

% comments
\newcommand{\lukas}[1]{\todo[inline, color=blue!20]{LW: #1}}
\newcommand{\huseyin}[1]{\todo[inline, color=red!20]{HI: #1}}
\newcommand{\rob}[1]{\todo[inline, color=green!20]{RS: #1}}
\newcommand{\sahar}[1]{\todo[inline, color=orange!20]{SA: #1}}
\newcommand{\eric}[1]{\todo[inline, color=purple!20]{EL: #1}}
\newcommand{\jana}[1]{\todo[inline, color=yellow!20]{JK: #1}}

\newcommand{\robinline}[1]{\textbf{\color{green} RS: #1}}

% table
\usepackage{colortbl}
\usepackage{multirow}
\usepackage{array}

% algo
\usepackage{algorithm}
\usepackage{algorithmic}

% For theorems and such
\usepackage{amsmath}
% \usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{dsfont}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}



==> papers/contextual_integrity/rebuttal.tex <==
\section*{Rebuttal}

%%%%%%%%%%%%%% I use the Markdown format for Openreview comments in the Rebuttal section. %%%%%%%%%%%%%%

% We can submit a summary to the chairs (or the AC) after rebuttal, which may help on their final decisions.
% \subsection*{Summary}

% Dear Chairs,

% We greatly appreciate your time spent handling our paper. 
% We have addressed all the reviewers' questions. 
% We briefly summarize the discussion here, and hope this would help with the evaluation.

% --

% 1. Reviewer ``b5NE``



% --

% 2. Reviewer ``rrV6``



% --

% 3. Reviewer ``y7VK``



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{Reviewer b5NE, Rating: 4, Confidence: 3}

\textbf{Response to W1:} \textit{“The reward function is somewhat arbitrary. Other than filtering for keywords, would it be better to learn a reward model, or use a prompted LLM to generate the reward?”}

\textcolor{red}{No need to modify.}

We thank the reviewer for this insightful suggestion. We chose a rule-based reward function based on keyword presence due to several practical and methodological considerations:

\begin{itemize}[left=0pt]
\item \textbf{Effectiveness and Precision:} Our rule-based reward function directly assesses whether required information is present and restricted information is omitted. This provides a precise and interpretable training signal aligned with the contextual integrity (CI) framework. As shown in Table~1 and Table~3, this reward structure leads to consistent improvements across our metrics and to the external PrivacyLens benchmark.

\item \textbf{Efficiency and Simplicity:} Rule-based rewards are computationally efficient and require no additional supervision or inference during training, unlike reward models or LLM judges which introduce significant overhead in GPU memory, inference time, and token price.

\item \textbf{Robustness Against Reward Hacking:} Learned reward models and LLM-based judges can be susceptible to \emph{reward hacking}, where models learn to exploit weaknesses in the reward mechanism rather than truly learning CI principles. They may also introduce inconsistency and drift, especially when CI violations are subtle or context-dependent.

\item \textbf{Controlled Evaluation Setting:} Since our synthetic dataset is automatically annotated with ground truth regarding required and restricted information, we are in a strong position to define unambiguous, high-quality reward signals without relying on approximations. First, we can easily control the filtering keywords depending on scenarios. Second, we can control the integrity-utility metrics depending on requirements as shown in Table~4.

\end{itemize}

That said, we agree that reward learning or prompting-based supervision could be promising directions for future work, particularly in settings where there is an abundance of high-quality data to train a reliable reward model or to construct a rubric-based LLM judge that mitigates potential reward hacking.


\textbf{Response to Q1:} \textit{“In Table 2, DeepSeek-R1-Distill-Qwen-14B originally has higher utility than the instruction-tuned Qwen 14B, but after RL training the utility lowered significantly. This much decrease due to RL is not seen in the IT models in Table 1. What could be happening?”}

\textcolor{red}{Added in Appendix \ref{app:Additional_Discussions}.}

We thank the reviewer for this thoughtful observation. The key reason lies in the initial behavior of the DeepSeek-R1-Distill-Qwen-14B model prior to RL training. As shown in Table~2, this model tends to disclose \emph{all} information - both required and restricted attributes - in its outputs. This behavior yields very high utility scores but results in low integrity and complete scores. In the extreme case, a model that always reveals all attributes would achieve $100\%$ utility but $0\%$ integrity and complete.

After applying CI-RL, the model learns to withhold restricted attributes, which leads to significant improvements in both integrity and complete metrics. However, this shift in behavior naturally causes a modest drop in utility, as the model becomes more cautious overall.

In contrast, the instruction-tuned (IT) models in Table~1 start from a more balanced behavior: they do not aggressively disclose all available information, and thus have relatively higher integrity and complete scores even before RL. Because their initial utility is lower (due to more conservative sharing), RL training can improve CI adherence while maintaining or even slightly improving utility.

As an additional point regarding the initial behavior of the DeepSeek-R1-Distill-Qwen-14B model, we note that DeepSeek-R1-Distill-Qwen-14B is primarily optimized for reasoning in scientific and technical domains at the expense of broader domain coverage, whereas our synthetic dataset covers diverse, real-world contexts (e.g., hospitality, education, family) that may fall outside its distributional strengths. This domain mismatch could further contribute to the model’s lower task completion performance under CI constraints initially.


\textbf{Response to W2 and Q2:}\textit{“only does evaluation on the PrivacyLens dataset.”} and \textit{“Could you also compare to the dataset in [1]?”}

\textcolor{red}{Added in Appendix \ref{sec:supplementary_results}.}

We thank the reviewer for this suggestion. We would like to begin by explaining in detail why we chose to evaluate on the PrivacyLens benchmark in this work.

As noted by [2], ConfAIde primarily consists of probing-style questions and focuses on a single application: meeting summarization and action-item generation, with only $20$ test cases. Moreover, it does not explicitly model the agentic context.

In contrast, PrivacyLens spans diverse tasks across multiple domains and agent roles, with rich scenarios and fine-grained annotations designed to reflect realistic interactions in agentic deployments. It includes approximately $500$ test cases and supports evaluation of dynamic, multi-turn interactions between users and assistants.

Given these differences, we believe PrivacyLens offers a more comprehensive and modern evaluation framework for studying contextual integrity (CI) in LLMs, particularly in settings that closely mirror practical deployments.

However, in response to the reviewer’s suggestion, we have additionally evaluated our CI-RL-trained Qwen2.5-7B-Instruct model on the ConfAIde benchmark. While our primary evaluation focused on PrivacyLens for the reasons outlined above, we recognize the value of broader comparison and made a concerted effort to ensure compatibility with ConfAIde’s format and evaluation setup. Our results show that CI-RL also leads to meaningful improvements on ConfAIde, further validating the generality of our approach.

\begin{table}[h]
    \centering
    \caption{Pearson’s correlation between human and model judgments for Tier 1, Tier 2.a, and Tier 2.b, higher values show more agreement.}
    \begin{tabular}{lc|cc|cc|cc}
        \toprule
        \multicolumn{2}{l}{Model} & \multicolumn{2}{|c}{Tier 1 $\uparrow$} &  \multicolumn{2}{c}{Tier 2.a $\uparrow$} & \multicolumn{2}{c}{Tier 2.b $\uparrow$} \\
        \midrule
        Qwen2.5-7B-Instruct & \color{PineGreen}{+ \textbf{CI-RL}} & 0.58 & \color{PineGreen}{\textbf{0.67}} & 0.51 & \color{PineGreen}{\textbf{0.69}} & 0.48 & \color{PineGreen}{\textbf{0.48}} \\
        \bottomrule
    \end{tabular}
\label{tab:confaide1-r1}
\end{table}
% **Table 5:** Pearson’s correlation between human and model judgments for Tier 1, Tier 2.a, and Tier 2.b, higher values show more agreement.
% | Model                                  | Tier 1 &uarr;         | Tier 2.a &uarr;       | Tier 2.b &uarr;       |
% | :------------------------------------- | :--------------------: | :--------------------: | :--------------------: |
% | Qwen2.5-7B-Instruct  &nbsp; **+CI-RL** | 0.58  &nbsp; **0.67** | 0.51  &nbsp; **0.69** | 0.48  &nbsp; **0.48** |

Table~\ref{tab:confaide1} demonstrates that our CI-RL approach leads to improved correlation between human and model judgments across Tier 1 and Tier 2, which evaluates the basic ability to understand the sensitivity of a given information and expectations of information flow within context.

\begin{table}[h]
    \centering
    \caption{Results for Tier 3: Theory of mind as context. The leakage rate of model generations for contextually appropriate responses and handling private information within a more nuanced scenario involving three parties.}
    \begin{tabular}{lc|cc}
        \toprule
        \multicolumn{2}{l}{Model} & \multicolumn{2}{|c}{Leakage thru. string match $\downarrow$} \\
        \midrule
        Qwen2.5-7B-Instruct & \color{PineGreen}{+ \textbf{CI-RL}} & 0.91 & \color{PineGreen}{\textbf{0.52}}  \\
        \bottomrule
    \end{tabular}
\label{tab:confaide2-r1}
\end{table}
% **Table 6:** Results for Tier 3: Theory of mind as context. The leakage rate of model generations for contextually appropriate responses and handling private information within a more nuanced scenario involving three parties.
% | Model                                  | Leakage thru. string match &darr; |
% | :------------------------------------- | :---------------: |
% | Qwen2.5-7B-Instruct  &nbsp; **+CI-RL** | 0.91  &nbsp; **0.52** |

In the next tier (Tier 3), the evaluation focuses on the model’s ability to regulate the disclosure of private information in more complex, multi-party scenarios. Unlike the earlier tiers, which primarily assess a model's capacity to judge the appropriateness of given information flows, this tier examines whether the model can generate contextually appropriate responses that demonstrate an implicit understanding of others' perspectives—an ability related to theory of mind.
Once again, as shown in Table~\ref{tab:confaide2}, our CI-RL approach yields a substantial reduction in the leakage of private information in the model’s responses.

\begin{table}[h]
    \centering
    \caption{Results for Tier 4: Private and public information flow. The metrics evaluate the privacy reasoning of LLMs in terms of their ability
to discern private (leaks secret) and public information (omits info), when presented with both types in a single scenario. Lower is better for all metrics.}
    \begin{tabular}{lc|cc|cc|cc}
        \toprule
        \multicolumn{2}{l}{Model} & \multicolumn{2}{|c}{Leaks Secret $\downarrow$} &  \multicolumn{2}{c}{Omits Info $\downarrow$} & \multicolumn{2}{c}{Leaks Secret or Omits Info $\downarrow$} \\
        \midrule
        Qwen2.5-7B-IT & \color{PineGreen}{+ \textbf{CI-RL}} & 0.80 & \color{PineGreen}{\textbf{0.30}} & 0.10 & \color{PineGreen}{\textbf{0.15}} & 0.85 & \color{PineGreen}{\textbf{0.45}} \\
        \bottomrule
    \end{tabular}
\label{tab:confaide3-r1}
\end{table}
% **Table 7:** Results for Tier 4: Private and public information flow. The metrics evaluate the privacy reasoning of LLMs in terms of their ability to discern private (leaks secret) and public information (omits info), when presented with both types in a single scenario. Lower is better for all metrics.
% | Model                                  | Leaks Secret &darr;         | Omits Info &darr;       | Leaks Secret or Omits Info &darr; |
% | :------------------------------------- | :--------------------: | :--------------------: | :--------------------: |
% | Qwen2.5-7B-Instruct  &nbsp; **+CI-RL** | 0.80  &nbsp; **0.30** | 0.10  &nbsp; **0.15** | 0.85  &nbsp; **0.45** |

Table~\ref{tab:confaide3} reports the results of the metrics where models are used as AI meeting assistants generating a meeting summary, in which it is important to exclude a particular sensitive information from the discussion, while including the vital public information.
Finally, we observe that our CI-RL approach significantly improves task completion while adhering to CI constraints - reducing the rate of completions that either leak a secret or omit required information from $0.85$ to $0.45$.



\textbf{Summary:} 
We answer the questions about reward function, DeepSeek-R1-Distill-Qwen-14B model, and evaluate the performance on the ConfAIde [1] benchmark.
We hope our responses would address the concerns, and truly appreciate the re-evaluation.


[1] Mireshghallah et al. "Can LLMs Keep a Secret? Testing Privacy Implications of Language Models via Contextual Integrity Theory." ICLR 2024.

[2] Shao et al. "PrivacyLens: Evaluating Privacy Norm Awareness of Language Models in Action." NeurIPS 2024.

% [2] Jason Wei. "Asymmetry of verification and verifier’s law." https://www.jasonwei.net/blog/asymmetry-of-verification-and-verifiers-law




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{Reviewer rrV6, Rating: 5, Confidence: 5}

\textbf{Response to W1:} \textit{“It’d be good to have some stats for the dataset you generate to show its diversity and balance. For example, in the prompt on page 21 (and also in line 157), you include a plan for avoiding obvious cues. Have you verified that those instructions were followed in the creation of the dataset?”}

\textcolor{red}{Added in Appendix \ref{sec:append_Hyperparameters}.}

We thank the reviewer for highlighting this important point. While our main focus was on evaluating contextual integrity under controlled conditions, we agree that providing a quantitative overview of our synthetic dataset would enhance transparency. In the following, we provide a summary of key dataset statistics.

%---------------------------  DATASET STATISTICS  ---------------------------
\begin{table}[h]
\centering
\small
\caption{Statistics of our \textbf{synthetic dataset} ($n=729$).}
\label{tab:data-stats_r2}
\begin{tabular}{lrr}
\toprule
\textbf{Application Domain} & \textbf{\#} & \textbf{\%} \\
\midrule
Healthcare      & 143 & 19.6 \\
Hospitality     & 100 & 13.7 \\
Family          &  87 & 11.9 \\
Education       &  78 & 10.7 \\
Finance         &  74 & 10.2 \\
Entertainment   &  73 & 10.0 \\
Friends         &  69 &  9.5 \\
Government      &  67 &  9.2 \\
eCommerce       &  38 &  5.2 \\
\midrule
\textbf{Privacy Principle} & & \\
Confidentiality & 428 & 58.7 \\
Proportionality & 201 & 27.6 \\
Consent         & 100 & 13.7 \\
\bottomrule
\end{tabular}
\end{table}
% | Application Domain |   \# |   \% |
% | :--------------------- | -------: | -------: |
% | Healthcare              | 143 | 19.6 |
% | Hospitality              | 100 | 13.7 |
% | Family                    | 87  | 11.9 |
% | Education              | 78  | 10.7 |
% | Finance                  | 74  | 10.2 |
% | Entertainment        | 73  | 10.0 |
% | Friends                  | 69  | 9.5 |
% | Government          | 67  | 9.2 |
% | eCommerce          | 38  | 5.2 |
% | **Privacy Principle**   |     |     |
% | Confidentiality       | 428 | 58.7 |
% | Proportionality      | 201 | 27.6 |
% | Consent                | 100 | 13.7 |

\begin{table}[h]
\centering
\small
\caption{Size of the \emph{allowed} vs.\ \emph{disallowed} attribute
lists per example and the vocabulary covered by the entire dataset.}
\label{tab:attr-stats_r2}
\begin{tabular}{lrrrrrrr}
\toprule
& \textbf{Min} & \textbf{Max} & \textbf{Mean} & \textbf{Median} & \textbf{Unique} \\
\midrule
Allowed     & 1 & 5 & 2.73 & 3 & 526 \\
Disallowed  & 1 & 3 & 2.08 & 2 & 322 \\
\bottomrule
\end{tabular}
\end{table}
% |            | Min | Max | Mean | Median | Unique |
% | :--------- | --: | --: | ---: | -----: | -----: |
% | Allowed    | 1   | 5   | 2.73 | 3      | 526    |
% | Disallowed | 1   | 3   | 2.08 | 2      | 522    |

\paragraph{Take‑away.}
The dataset spans \textbf{9} applications and \textbf{3} privacy principles, with no extreme imbalance.
Each synthetic instruction includes on average \textbf{2.73} allowed and
\textbf{2.08} disallowed personal attributes, drawn from
\textbf{526} and \textbf{322} unique attribute types respectively,
illustrating substantial lexical diversity and coverage.

Regarding the verification of instructions for avoiding obvious cues, we conducted a manual audit of randomly sampled instances, and found that they adhere to CI expectations and scenario consistency.

\textbf{Response to W2:} \textit{“Appendix A should explain helpfulness, LR, and ALR. It mentions PrivacyLens before the paper gets (chronologically) to Section 5. Maybe a reference in the Appendix back to that section is already good enough.”}

\textcolor{red}{Added in Appendix \ref{sec:supplementary_results}.}

We truly thank the reviewer for this suggestion that would improve the overall clarity and navigability of the paper.

We will explain helpfulness, LR, and ALR with a reference back to Section 5 in Appendix A to enhance readability.



\textbf{Response to Q1:} \textit{“What happens in agentic scenarios where they’re using tools instead of tags (e.g., \texttt{<think>...</think>})? I think CI-CoT would be easy to adapt, but what about CI-RL?”}

We thank the reviewer for this insightful question. We agree that CI-CoT is relatively easy to adapt to tool-based agentic setups, since its logic applies to intermediate reasoning steps regardless of whether they are expressed via tags or function calls.

For CI-RL, we believe a similar structure can be adopted in tool-use scenarios. Specifically, the reasoning phase can occur within \texttt{<think>} tags, and the tool invocation can be explicitly marked with \texttt{<action>} tags or equivalent structured representations. Our rule-based reward function can then be applied to these spans—assessing whether restricted information is leaked or required information omitted in action segments. This setup would preserve the modularity of our current approach and make it possible to train for contextual integrity in tool-augmented agents.


\textbf{Response to Q2:} \textit{“What is the temperature used for the dataset generation? You reported it for training in Appendix F and for PrivacyLens in Section 5, but not for the dataset generation.”}

\textcolor{red}{Added in Appendix \ref{sec:supplementary_results}.}

We thank the reviewer for pointing out this omission. During synthetic dataset generation (Section~3), we used a decoding temperature of 0.7 to encourage diverse but coherent outputs. We will add this setting description in the revised version.


\textbf{Response to Q3:} \textit{“Lines 230–231: ‘The results demonstrate that instruction-tuned LLMs achieve substantially higher integrity, utility, and task completion scores compared to LRMs, even after CI-RL training.’ In my opinion, these results (before CI-RL) are comparable across LLM and LRM. It’s not a big deal, just mentioning it.”}

\textcolor{red}{Modified in Section \ref{sec:experiments}.}

We appreciate the reviewer’s observation. We agree that the differences in pre-RL performance between instruction-tuned LLMs and LRMs are not uniformly large across all metrics. We will change this statement more accurately in the revised version.


\textbf{Response to Q4:} \textit{“What is the trade-off in terms of the number of output tokens? This would increase the price, so it’d be good to know.”}

\textcolor{red}{Added in Appendix \ref{sec:append_Hyperparameters}.}

We appreciate the reviewer highlighting this practical consideration. We ran statistics on the number of output tokens produced by the CI-RL-trained model over the PrivacyLens benchmark. The distribution is as follows:

\begin{itemize}[left=0pt]
    \item \textbf{Minimum:} 60 tokens
    \item \textbf{Maximum:} 836 tokens
    \item \textbf{Mean:} 244.72 tokens
    \item \textbf{Standard deviation:} 126.44 tokens
\end{itemize}

These results suggest that while the output lengths vary with task complexity, the overall response length remains moderate. We note that our reward function does not explicitly encourage longer outputs; in fact, CI-RL often leads to more focused completions by discouraging unnecessary or privacy-violating content.

We have further conducted a statistical analysis of the correlation between the number of thinking tokens and both helpfulness and leakage scores. The correlations were weak in both cases, suggesting that longer chains of thought are not strongly associated with improved task performance or increased risk. This indicates that in this domain, lengthy reasoning traces may not be necessary — potentially offering cost advantages in agentic settings.


\textbf{Summary:}
We appreciate the reviewer's valuable feedback, including descriptions of the data and the metrics in the appendices, temperature for the data generation, rigorous descriptions on LRMs \& LLMs, and trade-off of output tokens, which significantly improve the quality of the paper.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{Reviewer y7VK, Rating: 2, Confidence: 2}


\textbf{Response to W1:} \textit{
    The method lacks innovation.
    The article constructs a dataset through a large model (GPT) and then trains a small model through reinforcement learning.
    In essence, it is just a simple knowledge distillation.
    Moreover, the final experiment in Table 3 shows that the performance of the trained small model does not reach the level of the baseline model without the CoT prompt, which shows that the method in this article still has a lot of room for improvement.
}

\textcolor{red}{No need to modify.}


We thank the reviewer for raising this concern and welcome the opportunity to clarify the key contributions of our work and the interpretation of Table~3.

While our approach does leverage large models (GPT), their role is limited to the initial setup of contextual integrity (CI) — specifically, for generating scenarios, attributes, and user requests. We believe this is fundamentally different from standard knowledge distillation pipelines, which typically require access to teacher model outputs (e.g., logits, soft labels, or full demonstrations). In contrast, our method trains smaller models via RL using a reward function that encodes privacy constraints — without relying on privileged supervision or guidance from a stronger model. Therefore, we do not access model logits, soft labels, or demonstrations from Claude, Gemini, or GPT models during training.

The core innovation lies in how we formulate **contextual integrity (CI) as a RL problem** and design a **rule-based reward signal** that can guide small models to internalize abstract, high-level norms about information flow. This makes our method more interpretable, extensible, and efficient than black-box imitation from GPT outputs. Moreover, we demonstrate CI-RL is effective across diverse model families and privacy benchmarks, which, to our knowledge, has not been done before.

We believe the confusion regarding Table~3 may stem from presentation. The section titled “Baseline LLMs” reports results from large, proprietary models (e.g., Claude, Gemini), while the “Open Weights (ours)” section contains models we trained using CI-RL, starting from open checkpoints. These groups are intended to provide complementary reference points — not a direct distillation lineage. We will revise the table caption and surrounding text to better clarify this separation and avoid confusion.

Importantly, the fact that our CI-RL-trained open-weight models approach the performance of larger closed LLMs highlights the effectiveness of our approach without relying on privileged supervision. This demonstrates a viable path for low-cost, CI respecting LLM deployment using open models.

--

\textbf{Response to W2:} \textit{
    The dataset is relatively small (only 700 examples), which may not cover different domains and more complex scenarios.
    Moreover, the dataset is generated using GPT without human annotators, which may induce model bias.
    How to ensure the correctness and rationality of the generated dataset?
}

\textcolor{red}{No need to modify.}

We thank the reviewer for raising this important point regarding dataset quality and coverage.

\textbf{Dataset Size and Domain Coverage.} While the training dataset contains 700 examples, it is used specifically to fine-tune models via RL on CI constraints — not to train a model from scratch. We found this scale sufficient to shape model behavior under our reward function. Moreover, our test-time evaluations are conducted on the significantly broader PrivacyLens benchmark (500+ held-out test cases), which spans diverse domains and interaction types. This provides strong external validation of generalization beyond the training distribution. In fact, we view the ability to achieve strong CI performance using only 700 training examples as a key strength of our approach. It underscores the sample efficiency and scalability of CI-RL — demonstrating that meaningful generalization can be attained without large-scale annotation or privileged supervision. We believe this result is not a limitation but a promising signal that our method can be deployed efficiently in real-world settings.

\textbf{Correctness and Bias Control.} To ensure the quality of the synthetic dataset, we adopted several precautions during generation:
\begin{itemize}[left=0pt]
    \item Prompts were carefully designed to avoid obvious cues or shortcut signals (e.g., keyword repetition), as discussed in Section~3.
    \item We incorporated randomized role, domain, and attribute sampling to increase diversity and reduce prompt-template artifacts.
    \item We conducted a manual audit with randomly sampled instances, and found that over they adhere to CI expectations and scenario consistency.
\end{itemize}

While we completely agree with the reviewer that large-scale, human-reviewed datasets spanning a broad range of domains and complex scenarios would be ideal — and would undoubtedly contribute to stronger, more reliable model deployments — we emphasize that our goal in this work is different. We aim to demonstrate that even in the absence of extensive human annotation, one can make meaningful progress toward CI-aligned model behavior by leveraging formal definitions and scalable, programmatic supervision. We designed our method to be cost-efficient, reproducible, and bootstrappable, and we view the integration of human feedback as a highly promising direction for future work.


--

\textbf{Response to W3:} \textit{
    The experiment only tests on the synthesized dataset and PrivacyLens, which is insufficient to show the outperformance of the method.
    It is suggested to test on a more realistic and comprehensive benchmark (such as CONFAIDE(ICLR24)) and compare with previous methods, such as AirGapAgent (CCS24).
}

\textcolor{red}{Added in Appendix \ref{sec:supplementary_results}.}

We thank the reviewer for this suggestion. We would like to begin by explaining in detail why we chose to evaluate on the PrivacyLens benchmark in this work.

As noted by [2], ConfAIde primarily consists of probing-style questions and focuses on a single application: meeting summarization and action-item generation, with only $20$ test cases. Moreover, it does not explicitly model the agentic context.

In contrast, PrivacyLens spans diverse tasks across multiple domains and agent roles, with rich scenarios and fine-grained annotations designed to reflect realistic interactions in agentic deployments. It includes approximately $500$ test cases and supports evaluation of dynamic, multi-turn interactions between users and assistants.

Given these differences, we believe PrivacyLens offers a more comprehensive and modern evaluation framework for studying CI in LLMs, particularly in settings that closely mirror practical deployments.

However, in response to the suggestion, we have additionally evaluated our CI-RL-trained Qwen2.5-7B-Instruct model on the ConfAIde benchmark. While our primary evaluation focused on PrivacyLens for the reasons outlined above, we recognize the value of broader comparison and made a concerted effort to ensure compatibility with ConfAIde’s format and evaluation setup. Our results show that CI-RL also leads to meaningful improvements on ConfAIde, further validating the generality of our approach.

\begin{table}[ht]
    \centering
    \caption{Pearson’s correlation between human and model judgments for Tier 1, Tier 2.a, and Tier 2.b, higher values show more agreement.}
    \begin{tabular}{lc|cc|cc|cc}
        \toprule
        \multicolumn{2}{l}{Model} & \multicolumn{2}{|c}{Tier 1 $\uparrow$} &  \multicolumn{2}{c}{Tier 2.a $\uparrow$} & \multicolumn{2}{c}{Tier 2.b $\uparrow$} \\
        \midrule
        Qwen2.5-7B-Instruct & \color{PineGreen}{+ \textbf{CI-RL}} & 0.58 & \color{PineGreen}{\textbf{0.67}} & 0.51 & \color{PineGreen}{\textbf{0.69}} & 0.48 & \color{PineGreen}{\textbf{0.48}} \\
        \bottomrule
    \end{tabular}
\end{table}
% **Table 5:** Pearson’s correlation between human and model judgments for Tier 1, Tier 2.a, and Tier 2.b, higher values show more agreement.
% | Model                                  | Tier 1 &uarr;         | Tier 2.a &uarr;       | Tier 2.b &uarr;       |
% | :------------------------------------- | :--------------------: | :--------------------: | :--------------------: |
% | Qwen2.5-7B-Instruct  &nbsp; **+CI-RL** | 0.58  &nbsp; **0.67** | 0.51  &nbsp; **0.69** | 0.48  &nbsp; **0.48** |

Table~\ref{tab:confaide1} demonstrates that our CI-RL approach leads to improved correlation between human and model judgments across Tier 1 and Tier 2, which evaluates the basic ability to understand the sensitivity of a given information and expectations of information flow within context.

\begin{table}[ht]
    \centering
    \caption{Results for Tier 3: Theory of mind as context. The leakage rate of model generations for contextually appropriate responses and handling private information within a more nuanced scenario involving three parties.}
    \begin{tabular}{lc|cc}
        \toprule
        \multicolumn{2}{l}{Model} & \multicolumn{2}{|c}{Leakage thru. string match $\downarrow$} \\
        \midrule
        Qwen2.5-7B-Instruct & \color{PineGreen}{+ \textbf{CI-RL}} & 0.91 & \color{PineGreen}{\textbf{0.52}}  \\
        \bottomrule
    \end{tabular}
\end{table}
% **Table 6:** Results for Tier 3: Theory of mind as context. The leakage rate of model generations for contextually appropriate responses and handling private information within a more nuanced scenario involving three parties.
% | Model                                  | Leakage thru. string match &darr; |
% | :------------------------------------- | :---------------: |
% | Qwen2.5-7B-Instruct  &nbsp; **+CI-RL** | 0.91  &nbsp; **0.52** |

In the next tier (Tier 3), the evaluation focuses on the model’s ability to regulate the disclosure of private information in more complex, multi-party scenarios. Unlike the earlier tiers, which primarily assess a model's capacity to judge the appropriateness of given information flows, this tier examines whether the model can generate contextually appropriate responses that demonstrate an implicit understanding of others' perspectives—an ability related to theory of mind.
Once again, as shown in Table~\ref{tab:confaide2}, our CI-RL approach yields a substantial reduction in the leakage of private information in the model’s responses.

\begin{table}[ht]
    \centering
    \caption{Results for Tier 4: Private and public information flow. The metrics evaluate the privacy reasoning of LLMs in terms of their ability
to discern private (leaks secret) and public information (omits info), when presented with both types in a single scenario. Lower is better for all metrics.}
    \begin{tabular}{lc|cc|cc|cc}
        \toprule
        \multicolumn{2}{l}{Model} & \multicolumn{2}{|c}{Leaks Secret $\downarrow$} &  \multicolumn{2}{c}{Omits Info $\downarrow$} & \multicolumn{2}{c}{Leaks Secret or Omits Info $\downarrow$} \\
        \midrule
        Qwen2.5-7B-IT & \color{PineGreen}{+ \textbf{CI-RL}} & 0.80 & \color{PineGreen}{\textbf{0.30}} & 0.10 & \color{PineGreen}{\textbf{0.15}} & 0.85 & \color{PineGreen}{\textbf{0.45}} \\
        \bottomrule
    \end{tabular}
\end{table}
% **Table 7:** Results for Tier 4: Private and public information flow. The metrics evaluate the privacy reasoning of LLMs in terms of their ability to discern private (leaks secret) and public information (omits info), when presented with both types in a single scenario. Lower is better for all metrics.
% | Model                                  | Leaks Secret &darr;         | Omits Info &darr;       | Leaks Secret or Omits Info &darr; |
% | :------------------------------------- | :--------------------: | :--------------------: | :--------------------: |
% | Qwen2.5-7B-Instruct  &nbsp; **+CI-RL** | 0.80  &nbsp; **0.30** | 0.10  &nbsp; **0.15** | 0.85  &nbsp; **0.45** |

Table~\ref{tab:confaide3} reports the results of the metrics where models are used as AI meeting assistants generating a meeting summary, in which it is important to exclude a particular sensitive information from the discussion, while including the vital public information.
Finally, we observe that our CI-RL approach significantly improves task completion while adhering to CI constraints - reducing the rate of completions that either leak a secret or omit required information from $0.85$ to $0.45$.

[1] Mireshghallah et al. "Can LLMs Keep a Secret? Testing Privacy Implications of Language Models via Contextual Integrity Theory." ICLR 2024.

[2] Shao et al. "PrivacyLens: Evaluating Privacy Norm Awareness of Language Models in Action." NeurIPS 2024.


\textcolor{red}{Added in Appendix \ref{app:Additional_Discussions}.}

\textbf{Comparing with AirGapAgent (CCS24).}  We thank the reviewer for bringing it up, which we regard as a valuable and timely contribution to the study of privacy-aware LLM agents. AirGapAgent restricts access to private information by prompting an off-the-shelf LLM to decide which inputs are strictly necessary for task completion. In this sense, it shares conceptual similarities with our CI-CoT prompting approach, where a model reasons explicitly about which attributes to use or withhold based on CI.

While we agree that a more direct comparison would be informative, it is unfortunately not feasible at this time. To the best of our knowledge, neither the code nor the dataset for AirGapAgent has been released, and the paper does not report results on standardized benchmarks such as PrivacyLens or ConfAIde. This makes a head-to-head comparison under controlled conditions difficult.

Nonetheless, we view our work as complementary: AirGapAgent enforces privacy via task-specific prompting to limit information exposure, while our work focuses on training models — via both prompting (CI-CoT) and reinforcement learning (CI-RL) — to internalize generalizable CI norms. We are happy to discuss AirGapAgent in more detail in the related work section to highlight these connections and distinctions.

--

\textbf{Response to W4:} \textit{Privacy norms may be context-dependent and change over time, and the authors do not consider these effects. Additionally, some users may wish to insert custom rules and specifications, which are not supported by this document.}

\textcolor{red}{No need to modify.}

We appreciate the reviewer’s insightful observations. We fully agree that privacy norms are often context-dependent and can evolve over time, and that supporting user-specified rules would enhance practical deployment. 
First of all, our CI-CoT approach uses inference-time computation to reason about CI.
As a result, it can be adapted to different contexts and norms at inference time.
This enables flexibility in handling varying privacy norms and user-specific rules.
On the other hand, while our CI-RL approach adopts a fixed rule-based reward derived from CI, the design is intentionally modular and interpretable. 
This makes it straightforward to extend: adapting to evolving norms could be achieved by updating the rule definitions, and user-defined policies could be incorporated via additional constraints or templates during reward computation.
Because our approach does not rely on opaque learned reward models, we believe it offers a flexible foundation for incorporating such customization with minimal retraining.

We will highlight this extensibility more explicitly in Section~7 as an important direction for future work.


--

\textbf{Response to W5:} \textit{The paper did not include baselines in the evaluations. It is suggested to compare with different fine-tuning methods, such as PPO, SFT, and fine-tuning-free methods like few-shot prompts, etc.
}

\textcolor{red}{No need to modify.}

We thank the reviewer for this suggestion and would like to clarify that our evaluation does include a diverse set of baselines:

\begin{itemize}[left=0pt]
    \item \textbf{Open Weights baselines:} We evaluate several instruction-tuned models (e.g., from Mistral, Llama, Qwen model families) that have been trained via supervised fine-tuning (SFT) on general-purpose tasks.
    \item \textbf{Prompt-based baselines:} Our CI-CoT prompting approach is a fine-tuning-free method that inserts explicit reasoning steps to encourage CI respecting behavior without modifying model parameters.
    \item \textbf{Closed LLMs:} We additionally report results from powerful LLMs (e.g., Claude, Gemini) to situate the performance of our open-weight CI-RL models.
\end{itemize}

We appreciate the reviewer’s suggestion to include a comparison to SFT. We agree that SFT is a widely used method for behavior shaping in LLMs, but note that comparing it to reinforcement learning (RL) in the context of CI is not straightforward and opens up a number of important design choices.

In particular, effective SFT requires access to ground truth demonstrations of CI-respecting behavior. This raises the question of how such demonstrations should be obtained: via manual annotation (which is costly and not scalable), or by distilling from a stronger teacher model (which would shift the setting toward knowledge distillation). These decisions critically influence model behavior and fairness of comparison, and different choices could lead to vastly different outcomes. Exploring this space carefully is a substantial undertaking and, in our view, constitutes a promising direction for future work.

We also note that while fine-tuning-free methods such as few-shot prompting are appealing for their flexibility, they are unlikely to capture the full complexity of CI across diverse domains, roles, and interaction types. Few-shot examples may struggle to generalize to unseen scenarios or enforce subtle attribute-level privacy constraints without extensive manual curation. Our CI-CoT prompting approach is indeed a fine-tuning-free method—albeit using zero-shot prompting—and serves as a strong baseline in our evaluations. However, it is outperformed by our RL approach, which enables the model to internalize CI norms more robustly and generalize across a wider range of tasks.

Regarding PPO and related RL methods: we chose a simple rule-based reward with GRPO as the optimization algorithm for CI-RL. Our focus is not on comparing RL algorithms, but rather on demonstrating that even a simple, interpretable reward — derived from formal CI constraints — can guide model behavior effectively.

We appreciate the reviewer’s encouragement to explore additional tuning strategies and will consider deeper comparisons in future work.

% We add the PPO results. There is no significant difference in terms of evaluation performance. Thus, it shows the consistency of our pipeline with different optimizers. However, in the training process, GRPO is more memory efficient and only costs about $60-70\%$ of training time in PPO.

% For SFT, as there is no ground truth response data, it is not feasible to perform SFT without supervised responses. But it is feasible to perform RL, as the restricted and requested attributes is known.

% \begin{table}[!ht]
% \centering
% \caption{Method comparison with the Qwen2.5-7B-Instruct model.}
% \begin{tabular}{l|c|c|c}
% \toprule
% \multicolumn{1}{l}{Method} & \multicolumn{1}{|c}{$\mathcal{I}$ (in \%) $\uparrow$} & \multicolumn{1}{c}{$\mathcal{U}$ (in \%) $\uparrow$} & \multicolumn{1}{c}{$\mathcal{C}$ (in \%) $\uparrow$} \\
% \midrule
% IT & 46.9 & 62.5 & 29.7 \\
% % CI-CoT &  &  &  \\
% CI-GRPO & 75.0 & 67.2 & 48.4 \\
% CI-PPO &  &  &   \\
% \bottomrule
% \end{tabular}
% \label{tab:ppo_main}
% \end{table}

% \begin{table}[!ht]
% \centering
% \caption{Method comparison on PrivacyLens with the Qwen2.5-7B-Instruct model.}
% \begin{tabular}{l|c|c|c}
% \toprule
% \multicolumn{1}{l}{Method} & \multicolumn{1}{|c}{LR (in \%) $\downarrow$} & \multicolumn{1}{c}{ALR (in \%) $\downarrow$} & \multicolumn{1}{c}{Helpful [0-3] $\uparrow$} \\
% \midrule
% IT & 50.3 & 52.4 & 1.99 \\
% CI-CoT & 44.8 & 45.7 & 2.13 \\
% CI-GRPO & 33.7 & 33.9 & 2.08 \\
% CI-PPO &  &  &  \\
% \bottomrule
% \end{tabular}
% \label{tab:ppo_privacylens}
% \end{table}


--

\textbf{Appreciation and Closing Note:}



==> papers/contextual_integrity/sections/experiment_links.tex <==
\label{Sec:Experiments}

\subsection{Model type and size}
\begin{itemize}
    \item Qwen/Qwen2.5-1.5B-Instruct: \href{https://ml.azure.com/runs/sharp_drop_71dlk5s4x5?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
    \item Qwen/Qwen2.5-3B-Instruct: \href{https://ml.azure.com/runs/great_carrot_phrpj5wkvd?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
    \item Qwen/Qwen2.5-7B-Instruct: \href{https://ml.azure.com/runs/joyful_kitchen_x32f3f12z8?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47}{AML Link}
    \item Qwen/Qwen2.5-14B-Instruct: \href{https://ml.azure.com/runs/wheat_spring_s1w0xwk02h?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
    \item Qwen/Qwen2.5-32B-Instruct (gpu=0.5): \href{https://ml.azure.com/runs/silly_brick_q0ldc15h24?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
    \item Qwen/Qwen2.5-32B-Instruct (gpu=0.6): \href{https://ml.azure.com/runs/neat_rat_2t4ymffghx?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
    \item Qwen/Qwen2.5-32B-Instruct (original model): \href{https://ml.azure.com/experiments/id/7e4ee235-0c0e-4b0d-aee8-8b7cdfb8a59d/runs/witty_gyro_x5b9cn5dj3?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
    \item meta-llama/Llama-3.1-8B-Instruct: \href{https://ml.azure.com/runs/mighty_moon_m7k3y6192d?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
    \item deepseek-ai/DeepSeek-R1-Distill-Qwen-7B: \href{https://ml.azure.com/runs/jolly_stomach_zrg4sj0dj8?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
    \item mistralai/Mistral-7B-Instruct-v0.3: \href{https://ml.azure.com/runs/tidy_beard_3gnk1mz96j?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
\end{itemize}

\subsection{KL penalty}
\begin{itemize}
\item Qwen/Qwen2.5-7B-Instruct: \href{https://ml.azure.com/runs/blue_lettuce_g44glq3q6d?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{KL=0}
\item Qwen/Qwen2.5-7B-Instruct: \href{https://ml.azure.com/runs/affable_chain_k640y6zwqn?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{Previous AML Link, KL=0.001}
\item Qwen/Qwen2.5-7B-Instruct: \href{https://ml.azure.com/runs/icy_cushion_651v3cr2rr?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47}{PPO}
\item Qwen/Qwen2.5-7B-Instruct: \href{https://ml.azure.com/runs/red_camel_kzhs4s3x0s?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{KL=0.01}
\item Qwen/Qwen2.5-7B-Instruct: \href{https://ml.azure.com/runs/plucky_insect_xwc7njm0c7?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{KL=0.1}
\item Qwen/Qwen2.5-7B-Instruct: \href{https://ml.azure.com/runs/amusing_net_f5wqbljxt4?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{KL=1}
\item Qwen/Qwen2.5-7B-Instruct: \href{https://ml.azure.com/runs/jovial_wall_bkq6rn3xvm?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47}{KL=10}
\end{itemize}

\subsection{Utility-privacy trade-off with reward design}

\begin{itemize}
\item Qwen/Qwen2.5-7B-Instruct: \href{https://ml.azure.com/experiments/id/968e292d-bcae-4929-a163-0ecd7d45da84/runs/good_parsnip_4h4sd6js5q?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{Allowed=3, Disallowed=1}
\item Qwen/Qwen2.5-7B-Instruct: \href{https://ml.azure.com/runs/mango_deer_swtxsb1dn0?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47}{Allowed=2, Disallowed=1}
\item Qwen/Qwen2.5-7B-Instruct: \href{https://ml.azure.com/runs/affable_chain_k640y6zwqn?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{Previous AML Link, Allowed=1, Disallowed=1}
\item Qwen/Qwen2.5-7B-Instruct: \href{https://ml.azure.com/runs/frank_vulture_x5trbq9lyd?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47}{Allowed=1, Disallowed=2}
\item Qwen/Qwen2.5-7B-Instruct: \href{https://ml.azure.com/experiments/id/968e292d-bcae-4929-a163-0ecd7d45da84/runs/khaki_celery_bs39247fmg?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{Allowed=1, Disallowed=3}
\end{itemize}

\paragraph{Fixed global steps}
\begin{itemize}
\item Qwen/Qwen2.5-7B-Instruct: \href{https://ml.azure.com/experiments/id/968e292d-bcae-4929-a163-0ecd7d45da84/runs/good_flag_8dftjmlgxf?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{+1, -0.25}
\item Qwen/Qwen2.5-7B-Instruct: \href{https://ml.azure.com/experiments/id/968e292d-bcae-4929-a163-0ecd7d45da84/runs/red_brain_7kk0z1g18g?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{+1, -0.5}
\item Qwen/Qwen2.5-7B-Instruct: \href{https://ml.azure.com/runs/modest_pea_lg27z3yxzb?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47}{+1, -1}
\item Qwen/Qwen2.5-7B-Instruct: \href{https://ml.azure.com/experiments/id/968e292d-bcae-4929-a163-0ecd7d45da84/runs/careful_box_dbp572wjkx?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{+0.5, -1}
\item Qwen/Qwen2.5-7B-Instruct: \href{https://ml.azure.com/experiments/id/968e292d-bcae-4929-a163-0ecd7d45da84/runs/keen_school_wrxvbyv4ns?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{+0.25, -1}
\end{itemize}

% from version 1
% \subsection{Model type and size}
% Fix the RL algorithm as GRPO.
% \begin{itemize}
%     \item Qwen/Qwen2.5-1.5B: \href{https://ml.azure.com/runs/frosty_zebra_k3cr5gxl8z?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47}{AML Link}
%     \item Qwen/Qwen2.5-1.5B-Instruct: \href{https://ml.azure.com/runs/cyan_battery_8nz29rh142?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
%     \item Qwen/Qwen2.5-3B: \href{https://ml.azure.com/runs/olive_guava_dw5hy3ts7c?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
%     \item Qwen/Qwen2.5-3B-Instruct: \href{https://ml.azure.com/runs/lucid_corn_z3ybb7lff7?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
%     \item Qwen/Qwen2.5-7B: \href{https://ml.azure.com/runs/busy_floor_sgkcvjf9fz?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47}{AML Link}
%     \item Qwen/Qwen2.5-7B-Instruct: \href{https://ml.azure.com/runs/eager_tongue_3817nfw2m8?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47}{AML Link}
%     \item Qwen/Qwen2.5-14B: \href{https://ml.azure.com/runs/aeba64b1-048a-4dd4-a600-5d57077c5a4f?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47}{AML Link}
%     \item Qwen/Qwen2.5-14B-Instruct: \href{https://ml.azure.com/runs/goofy_boat_3gppnjg4tj?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47}{AML Link}
%     \item Qwen/Qwen2.5-32B: MAYBE
%     \item Qwen/Qwen2.5-32B-Instruct: MAYBE
% \end{itemize}

% \begin{itemize}
% \item meta-llama/Llama-3.1-8B: \href{https://ml.azure.com/runs/dynamic_raisin_xzqv277164?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
% \item meta-llama/Llama-3.1-8B-Instruct: \href{https://ml.azure.com/runs/nifty_star_nj798j5jcf?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
% \item mistralai/Mistral-7B-v0.3: \href{https://ml.azure.com/runs/hungry_cup_0v6kswb15l?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
% \item mistralai/Mistral-7B-Instruct-v0.3: \href{https://ml.azure.com/runs/bold_puppy_xqdj52mbfk?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47}{AML Link}
% \item mistralai/Ministral-8B-Instruct-2410: \href{https://ml.azure.com/runs/salmon_music_kmqdh3s7dd?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47}{AML Link}
% \end{itemize}



% \begin{itemize}
%     \item deepseek-ai/DeepSeek-R1-Distill-Qwen-1.5B: \href{https://ml.azure.com/runs/wheat_spade_fhjmslmc9q?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47}{AML Link}
%     \item deepseek-ai/DeepSeek-R1-Distill-Qwen-7B: \href{https://ml.azure.com/runs/plucky_chicken_t8lcjqnl16?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47}{AML Link}
%     \item deepseek-ai/DeepSeek-R1-Distill-Qwen-14B: HUSEYIN
%     \item deepseek-ai/DeepSeek-R1-Distill-Qwen-32B: MAYBE
% \end{itemize}

% \subsection{KL penalty}
% Fix the RL algorithm as GRPO and the model as Qwen/Qwen2.5-7B-Instruct and apply
% \begin{itemize}
%     \item KL penalty 0: \href{https://ml.azure.com/runs/neat_button_671vmh0ctx?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
%     \item KL penalty 0.001: \href{https://ml.azure.com/runs/eager_tongue_3817nfw2m8?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47}{AML Link} and \href{https://ml.azure.com/runs/tidy_pig_kqqhf5w16w?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47&monitoringView={%22options%22:{%22startTime%22:%222025-04-14T20:45:49.616Z%22,%22endTime%22:%222025-04-14T21:03:56.314Z%22}}}{Huseyin AML Link}
%     \item KL penalty 0.01: \href{https://ml.azure.com/runs/keen_papaya_jx7bvppvnj?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
%     \item KL penalty 0.1: \href{https://ml.azure.com/runs/ashy_chaconia_7cbn29qnlm?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
%     \item KL penalty 1.0: \href{https://ml.azure.com/runs/amusing_needle_j9pcgy0k5h?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
% \end{itemize}

% \subsection{Utility-privacy trade-off with reward design}
% Fix the model Qwen/Qwen2.5-7B-Instruct and apply
% \begin{itemize}
%     \item $\text{allowed} = +0.1, \text{disallowed} = -0.5$: \href{https://ml.azure.com/runs/eager_tongue_3817nfw2m8?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47}{AML Link}
%     \item $\text{allowed} = +0.2, \text{disallowed} = -0.4$: \href{https://ml.azure.com/experiments/id/2fe97015-e584-4842-81bd-b79228c1501c/runs/bold_rod_2hn8bwwrkb?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
%     \item $\text{allowed} = +0.3, \text{disallowed} = -0.3$: \href{https://ml.azure.com/experiments/id/2fe97015-e584-4842-81bd-b79228c1501c/runs/dreamy_wing_d948x09cx7?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
%     \item $\text{allowed} = +0.4, \text{disallowed} = -0.2$: \href{https://ml.azure.com/experiments/id/2fe97015-e584-4842-81bd-b79228c1501c/runs/olive_wheel_t5dh337dv7?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47}{AML Link}
%     \item $\text{allowed} = +0.5, \text{disallowed} = -0.1$: \href{https://ml.azure.com/runs/happy_lobster_7sph3nkzrk?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47}{AML Link}
% \end{itemize}

% \subsection{GRPO vs PPO}
% Fix the model Qwen/Qwen2.5-7B-Instruct and run GRPO and PPO five times each and compare metrics with confidence intervals.

% GRPO:
% \begin{enumerate}
%     \item Random seed $42$: \href{https://ml.azure.com/runs/eager_tongue_3817nfw2m8?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47}{AML Link}
% \end{enumerate}

% PPO:
% \begin{enumerate}
%     \item Random seed $42$: \href{https://ml.azure.com/experiments/id/2fe97015-e584-4842-81bd-b79228c1501c/runs/jovial_rose_7b7xv0yr2m?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{AML Link}
% \end{enumerate}


% \subsection{Prior Work}
% \begin{itemize}
%     \item Confaide: HUSEYIN, LUKAS, SAHAR
%     \item Privacy Lens: HUSEYIN, LUKAS, SAHAR
% \end{itemize}

\subsection{Academic Bench}
\begin{itemize}
    \item Qwen/Qwen2.5-1.5B-Instruct: \href{https://ml.azure.com/runs/sharp_drop_71dlk5s4x5?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{RL} \href{}{Origin}
    \item Qwen/Qwen2.5-3B-Instruct: \href{https://ml.azure.com/runs/great_carrot_phrpj5wkvd?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{RL} \href{https://ml.azure.com/runs/maroon_chaconia_qrwqgsf4n1?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{Origin}
    \item Qwen/Qwen2.5-7B-Instruct: \href{https://ml.azure.com/runs/joyful_kitchen_x32f3f12z8?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{RL} \href{https://ml.azure.com/runs/cyan_glass_5txmws0ptf?wsid=/subscriptions/acc09744-1ee3-4242-b375-93421c63af0c/resourcegroups/Singularity/workspaces/M365Research&tid=72f988bf-86f1-41af-91ab-2d7cd011db47#}{Origin}
    \item Qwen/Qwen2.5-14B-Instruct: \href{}{RL} \href{}{Origin}
\end{itemize}

==> papers/contextual_integrity/tables/academic_bench.tex <==
\begin{tabular}{c|cccccc}
\toprule[1.1pt]
% \hline
 {Method} & {IFEval$\uparrow$} & {GPQA$\uparrow$} & {MMLU$\uparrow$} & {HellaSwag$\uparrow$} & {TruthfulQA$\uparrow$} & {GSM8K$\uparrow$} \\
\midrule[1.1pt]
{Qwen2.5-1.5B-Instruct} & { } & { } & { } & { } & { } & { } \\
\rowcolor{gray!20} {+\textbf{CI-optimized RL}} & {42.1} & {25.9} & {59.3} & {67.9} & {37.2} & { } \\
{Qwen2.5-3B-Instruct} & {62.5} & {26.3} & {65.5} & {74.9} & {50.2} & { } \\
\rowcolor{gray!20} {+\textbf{CI-optimized RL}} & {51.6} & { } & { } & {} & { } & { } \\
{Qwen2.5-7B-Instruct} & { } & { } & { } & { } & { } & { } \\
\rowcolor{gray!20} {+\textbf{CI-optimized RL}} & { } & { } & { } & { } & { } & { } \\
{Qwen2.5-14B-Instruct} & { } & { } & { } & { } & { } & { } \\
\rowcolor{gray!20} {+\textbf{CI-optimized RL}} & { } & { } & { } & { } & { } & { } \\
\bottomrule[1.1pt]
\end{tabular}

==> papers/contextual_integrity/tables/kl.tex <==
% \begin{tabular}{l|ccc|ccc}
%     \toprule
%     $\beta$ & Complete $\uparrow$ & Utility $\uparrow$ & Privacy $\uparrow$ & LR $\downarrow$ & Adjusted LR $\downarrow$ & Avg. Helpfulness $\uparrow$ \\
%     \midrule
%     0 & 50.0 & 68.8 & 76.6 & 32.9 & 35.1 & 2.01 \\
%     0.001 & 48.4 & 67.2 & 75.0 & 33.7 & 33.9 & 2.08 \\
%     0.01 & 46.9 & 62.5 & 79.7 & 34.3 & 35.4 & 2.14 \\
%     0.1 & 46.9 & 70.3 & 65.6 & 44.0 & 47.0 & 2.05 \\
%     1 & 26.6 & 62.5 & 50.0 & 46.5 & 49.4 & 2.05 \\
%     \bottomrule
% \end{tabular}

\begin{tabular}{l|ccc|ccc}
    \toprule
    $\beta$ & $\mathcal{C}$ (in \%) $\uparrow$ & $\mathcal{U}$ (in \%) $\uparrow$ & $\mathcal{P}$ (in \%) $\uparrow$ & LR $\downarrow$ & Adjusted LR $\downarrow$ & Helpfulness [0-3] $\uparrow$ \\
    \midrule
    0 & 56.3 & 68.8 & 79.7 & 36.1 & 39.8 & 2.02 \\
    0.001 & 48.4 & 67.2 & 75.0 & 33.7 & 33.9 & 2.08 \\
    0.01 & 51.6 & 70.3 & 78.1 & 35.7 & 37.0 & 1.98 \\
    0.1 & 45.3 & 73.4 & 67.2 & 41.2 & 43.1 & 2.09 \\
    1 & 28.1 & 59.4 & 53.1 & 46.5 & 46.9 & 1.97 \\
    \bottomrule
\end{tabular}


==> papers/contextual_integrity/tables/privacylens.tex <==
\pgfplotstableread[col sep=comma]{results/privacylens.csv}\datatable

\pgfplotstabletypeset[
    columns={model, info_leakage_rate, adjusted_info_leakage_rate, average_helpfulness_score, binary_helpfulness_rate},
    col sep=comma,
    columns/model/.style={
	column name=Model,
	string type, % Explicitly set column type to string
	string replace*={qwen-cot}{Qwen CoT},
	string replace*={qwen-rl}{Qwen RL},
	string replace*={qwen-base}{Qwen Base},
    },
    columns/info_leakage_rate/.style={column name=LR $\downarrow$},
    columns/adjusted_info_leakage_rate/.style={column name=Adjusted LR $\downarrow$},
    columns/average_helpfulness_score/.style={column name=average helpfulness $\uparrow$},
    columns/binary_helpfulness_rate/.style={column name=binary helpfulness $\uparrow$},
    every head row/.style={before row=\toprule, after row=\midrule},
    every last row/.style={after row=\bottomrule}
]{\datatable}


% \begin{tabular}{l|ccc}
%     \toprule
%     Model & LR (in \%) $\downarrow$ & Adjusted LR (in \%) $\downarrow$ & Helpfulness [0-3] $\uparrow$\\
%     \midrule
%     \multicolumn{4}{c}{\textit{Baseline LLMs}} \\
%     \midrule
%     Claude 3.7 Sonnet & 30.4 & 35.9 & 2.49 \\
%     \rowcolor{gray!20}
%     + \textbf{CI-CoT prompt} & 23.1 & 25.4 & 2.69 \\
%     Gemini 2.5 Flash & 29.0 & 30.8 & 2.75 \\
%     \rowcolor{gray!20}
%     + \textbf{CI-CoT prompt} & 19.7 & 24.0 & 2.31 \\
%     \midrule
%     \multicolumn{4}{c}{\textit{Baseline LRMs}} \\
%     \midrule
%     Claude 3.7 Sonnet Thinking & 32.0 & 34.6 & 2.75 \\
%     \rowcolor{gray!20}
%     + \textbf{CI-CoT prompt} & 20.1 & 22.6 & 2.63 \\
%     Gemini 2.5 Pro & 37.3 & 38.2 & 2.84 \\
%     \rowcolor{gray!20}
%     + \textbf{CI-CoT prompt} & 25.3 & 26.9 & 2.72 \\
%     \midrule
%     \multicolumn{4}{c}{\textit{Open Weights}} \\
%     \midrule
%     Mistral-7B-Instruct-v0.3 & 47.9 & 52.1 & 1.78 \\
%     \rowcolor{gray!20}
%     + \textbf{CI-CoT prompt} & 28.8 & 46.6 & 1.17 \\
%     \rowcolor{gray!20}
%     + \textbf{CI-RL} & 31.2 & 29.6 & 1.84 \\
%     Qwen2.5-7B-Instruct & 50.3 & 52.4 & 1.99 \\
%     \rowcolor{gray!20}
%     + \textbf{CI-CoT prompt} & 44.8 & 45.7 & 2.13 \\
%     \rowcolor{gray!20}
%     + \textbf{CI-RL} & 33.7 & 33.9 & 2.08 \\
%     Llama-3.1-8B-Instruct & 18.2 & 38.9 & 1.05 \\
%     \rowcolor{gray!20}
%     + \textbf{CI-CoT prompt} & 21.3 & 31.5 & 1.29 \\
%     \rowcolor{gray!20}
%     + \textbf{CI-RL} & 18.5 & 29.4 & 1.18 \\
%     Qwen2.5-14B-Instruct & 52.9 & 51.2 & 2.37 \\
%     \rowcolor{gray!20}
%     + \textbf{CI-CoT prompt} & 42.8 & 44.4 & 2.27 \\
%     \rowcolor{gray!20}
%     + \textbf{CI-RL} & 33.9 & 34.4 & 2.30 \\
%     \bottomrule
% \end{tabular}

==> papers/contextual_integrity/tables/reward_function.tex <==
\begin{tabular}{l|ccc|ccc}
    \toprule
    ($\alpha$, $\gamma$) & $\mathcal{I}$ (in \%) $\uparrow$ & $\mathcal{U}$ (in \%) $\uparrow$ & $\mathcal{C}$ (in \%) $\uparrow$ & LR $\downarrow$ & ALR $\downarrow$ & Helpful [0-3] $\uparrow$ \\
    \midrule
    (1, 0.25) & 71.9 & 71.9 & 48.4 & 38.5 & 39.3 & 2.12 \\
    (1, 0.5) & 78.1 & 76.6 & 59.4 & 35.7 & 38.6 & 2.02 \\
    (1, 1) & 75.0 & 67.2 & 48.4 & 33.7 & 33.9 & 2.08 \\
    (0.5, 1) & 79.7 & 71.9 & 57.8 & 34.1 & 36.1 & 1.98 \\
    (0.25, 1) & 82.8 & 68.8 & 57.8 & 32.3 & 35.3 & 2.01 \\
    \bottomrule
\end{tabular}

==> papers/mappo/mappo_body_thesis.tex <==
\section{Introduction}
\label{Sec:Introduction}

Reinforcement Learning from Human Feedback (RLHF) has emerged as a general paradigm for aligning large language models (LLMs) with human preferences.  Pioneering work framed the problem as reinforcement learning (RL) on a reward model trained from group-wise comparisons, yielding notable improvements in summarization and dialogue~\citep{christiano2017deep, stiennon2020learning}. Subsequent systems such as InstructGPT~\citep{ouyang2022training} demonstrated that RLHF could scale to billion‑parameter models and substantially boost helpfulness and safety~\citep{lan2025contextual}. Despite its practical successes, RLHF still suffers from noisy feedback, reward-model misalignment, optimization instability, and computation inefficiency with high memory cost, which together hinder its scalability and reliability~\citep{casper2023open, dai2023safe, pan2022effects}.

Direct Preference Optimization (DPO)~\citep{dpo_neurips2023} reframes the preference learning with a Kullback–Leibler (KL) regularized objective as a log-odds objective, effectively turning the task into Maximum Likelihood Estimation (MLE) over pairwise comparisons: The model is trained to assign a higher likelihood to the preferred response than to the rejected, while staying close to a reference policy.
The MLE perspective accounts for the efficiency of DPO, as it eliminates the need for rollouts or value functions.
However, this formulation also introduces a fundamental limitation: It considers only the relative likelihoods within each pair, overlooking the absolute reward magnitude and any external prior knowledge~\citep{amini2024direct, d2025anchored}. 
As a result, the training signal in DPO is inherently local, bounded by pairwise comparisons, and lacks global calibration across examples.

\subsection{Challenge}
A fundamental limitation of MLE-based preference optimization lies in its purely relative nature: It focuses on maximizing the \emph{gap} between chosen and rejected responses, yet lacks a mechanism to anchor their absolute probabilities.
As training progresses, the MLE objective tends to suppress the likelihood of the rejected response rather than elevate that of the preferred one. Empirical investigations~\citep{pal2024smaug, rafailov2024r, tajwar2024preference,zhang2024negative} consistently show a simultaneous reduction in the absolute probabilities assigned to both preferred and rejected answers, resulting in abnormal output distributions.
This undesirable dynamic, empirically known as the \textit{squeezing effect}~\citep{ren2024learning}, undermines policy calibration and injects instability into generation. 
The issue is especially severe in near-tie cases (in Figure~\ref{fig:compare_MLE_MAP}), especially when models approach human-level performance~\citep{liu2024reward, guo2024todo}, where both responses are reasonable yet MLE still enforces an artificial separation, draining probability mass from the high-quality region of the output space. Motivated by this, the key question that this paper aims to address is:

%{\em How can prior reward knowledge be incorporated into preference optimization to improve language model alignment?}

{\em How can we improve language model alignment through a more principled training signal, instead of an oversimplified MLE pipeline?}

In this paper, we answer the above question by introducing Maximum-a-Posteriori Preference Optimization (MaPPO)~\citep{lan2025mappo}, a simple yet principled extension of DPO that injects data‑driven prior knowledge into preference training. 
MaPPO augments the standard maximum-likelihood objective with a lightweight MaP regularizer, an additional log‑prior scaled by a calibrated reward gap, which proportionally adjusts each update to the confidence difference between the preferred and rejected answers. 
Instead of the oversimplified binary classification in MLE, this mechanism curbs the excessive penalization of near‑tie pairs while preserving DPO’s one‑step closed form and computational efficiency.

Extensive experiments demonstrate that MaPPO delivers consistently stronger performance across three public alignment benchmarks: AlpacaEval 2.0, Arena-Hard, and MT-Bench. 
We evaluate MaPPO on multiple model families, including Llama-3, Qwen2.5, and Mistral, under multiple model sizes. 
Compared to DPO, MaPPO achieves absolute win-rate gains of $94.3\%$ on AlpacaEval and $37.1\%$ on Arena-Hard when fine-tuned on the Mistral-7B-Instruct model. 
Moreover, the proposed MaPPO is suitable for both offline and online settings. 
These results validate that a lightweight prior is sufficient to produce stronger and better-calibrated policies.
Furthermore, MaPPO is designed as a drop-in regularization module and seamlessly integrates with a broad spectrum of recent DPO variants, including Iterative-DPO~\citep{dong2024rlhf}, SimPO~\citep{meng2024simpo}, IPO~\citep{pmlr-v238-gheshlaghi-azar24a}, and CPO~\citep{xu2024contrastive}. 
In all cases, we observe consistent gains up to $31.3\%$ on Arena-Hard in alignment scores without requiring additional computation or changes to the optimization pipeline. 
This suggests that MaPPO serves as a robust and general enhancement strategy for advanced preference training pipelines.

\subsection{Summary of Contributions}
In summary, the main contributions of this work are as follows:
\begin{enumerate}[left=0pt]
    \item We propose MaPPO, a principled extension of Direct Preference Optimization, which incorporates data-driven prior reward estimates into a Maximum-a-Posteriori (MaP) objective.
    \item We demonstrate that MaPPO naturally supports both offline (e.g., DPO) and online (e.g., I-DPO) preference optimization.
    \item We show that MaPPO is compatible with and enhances existing DPO variants, including SimPO, IPO, and CPO. For all variants, no additional hyperparameter is needed.
    \item Empirical results across multiple model series and model sizes confirm consistent improvements in alignment performance on standard benchmarks, including MT-Bench, AlpacaEval 2.0, and Arena-Hard.
\end{enumerate}

\paragraph{Notations.}
We use $\sigma (\cdot)$ to denote the logistic (sigmoid) function $\sigma (x) = \frac{1}{1 + e^{-x}}$.
% $\mathds{1}_{[\mathrm{condition}]}$ is an indicator function, and the value is $1$ if the condition is true, and $0$ otherwise.
For preference pairs, $\textbf{y}_w$ denotes the \textit{chosen} (winning) response, while $\textbf{y}_l$ denotes the \textit{rejected} (losing) response.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}
\label{Sec:Related_Work}

\paragraph{Direct Preference Optimization and its Variants.}
Driven by the complexity of online RLHF algorithms~\citep{santacroce2023efficient, zheng2023secrets}, recent research has pivoted toward efficient offline preference optimization.
Direct Preference Optimization (DPO)~\citep{dpo_neurips2023} frames preference alignment as maximum-likelihood estimation (MLE) under the Bradley-Terry (BT) model~\citep{bradley1952rank}, while IPO~\citep{pmlr-v238-gheshlaghi-azar24a} generalizes this framework without the pointwise‑reward assumption. Further, CPO~\citep{xu2024contrastive} jointly optimizes the sequence likelihood and a contrastive reward to perform supervised fine-tuning (SFT) and alignment in one pass. 
KTO~\citep{ethayarajh2024model} extends the paradigm to single‑response feedback via prospect theoretic utility. 
Recent DPO variants, ORPO~\citep{hong-etal-2024-orpo}, R-DPO~\citep{park2024disentangling}, and SimPO~\citep{meng2024simpo}, further push performance by discarding the reference model or regularizing response length.
%ORPO~\citep{hong-etal-2024-orpo} drops the reference model by introducing a direct odds ratio loss, and R‑DPO~\citep{park2024disentangling} regularizes answer length to curb verbosity. SimPO~\citep{meng2024simpo} removes the reference model and adds length normalization for lighter training.
\cite{yang2025weightedreward} further introduces a weight hyperparameter to balance the influence of preference pairs from different policies. 
\cite{zhao2025rainbowpo} then aims to combine the previous PO methods into one cohesive objective. 
However, all DPO-style variants rely on MLE in the training process, which oversimplifies the tuning of preferred and unpreferred responses as a binary classification problem.
%In our work, we introduce prior knowledge into the objective to guide preference optimization, enabling the model to align more effectively, a dimension that previous studies have not explored.

\paragraph{Confidence Degeneration in DPO.}
%Previous works~\citep{pal2024smaug, rafailov2024r, tajwar2024preference} observe that during DPO training, the absolute confidence assigned to both the preferred response $\mathbf{y}_w$ and the rejected response $\mathbf{y}_l$ can gradually decrease. 
\citet{pal2024smaug} and \citet{tajwar2024preference} show analytically and empirically that the expected DPO gradient often decreases the log-likelihood of the preferred response $\mathbf{y}_w$ instead of increasing it, leading to a simultaneous shrinkage of both responses.
\citet{rafailov2024r} observe the same trend, attributing the drop to the expected log ratio between the optimized and reference models. By showing that this is equivalent to the non-negative KL divergence, they conclude that DPO training inevitably lowers the likelihood of the chosen response.
Nemotron-4 \citep{adler2024nemotron} constraints the DPO loss with the reward margin. However, no motivation or theoretical perspective is given. Moreover, it cannot be used in the online setting and is unable to enhance the other DPO variants.
%\citet{rafailov2024r} report the same trend and explain the drop by $\mathbb E_{\pi_\text{ref}}\left[\beta \log \pi^* - \beta \log \pi_\text{ref}\right] = -\beta \mathbb{D}_{KL} (\pi_\text{ref} || \pi^*)$: the positive KL divergence between the reference and learned policies forces the implicit reward to decline over time.
More recent analyses of the learning dynamics in \cite{ren2024learning} have identified a phenomenon termed the \textit{squeezing effect}, whereby DPO training aggressively drains probability mass from all responses except the most confident one, $\mathbf{y}^*= \arg\max_{i \in [V ]\setminus {\mathbf{y}_l}} \pi_\theta (\mathbf{y} = i)$, consequently funneling this mass towards $\mathbf{y}^*$. 
Our method utilizes prior knowledge to soften the downward pressure on the rejected response $\mathbf{y}_l$, it markedly mitigates the squeezing effect. 

\iffalse
\begin{table}[t]
\caption{Performances of preference optimization methods.}
\centering
 % \small
\label{table:complexity}
\begin{tabular}{cccc}
\toprule[1.1pt]
% \hline
{Methods} & {Online} & {Offline} & {Memory Cost} \\
\midrule[1.1pt]
\rowcolor{gray!10} \multicolumn{1}{c}{DPO \citep{dpo_neurips2023}} & {} & {} & {} \\
\rowcolor{gray!10} {} & {\multirow{-2}{*}{$\mathcal{O}({\epsilon}^{-4})$}} & {\multirow{-2}{*}{$\mathcal{O}({\epsilon}^{-3})$}} & {\multirow{-2}{*}{-}} \\
 \multicolumn{1}{c}{IPO \citep{pmlr-v238-gheshlaghi-azar24a}} & {} & {} & {} \\
{} & \multirow{-2}{*}{$\mathcal{O}({\epsilon}^{-3.5})$} & \multirow{-2}{*}{$\mathcal{O}({\epsilon}^{-2.5})$} &  \multirow{-2}{*}{-} \\
\rowcolor{gray!10} \multicolumn{1}{c}{ORPO \citep{hong-etal-2024-orpo}} & {} & {} & {} \\
\rowcolor{gray!10} {} & {\multirow{-2}{*}{$\mathcal{O}({\epsilon}^{-4})$}} & {\multirow{-2}{*}{$\mathcal{O}({\epsilon}^{-3})$}} & {\multirow{-2}{*}{-}} \\
\multicolumn{1}{c}{I-DPO \citep{dong2024rlhf}} & {} & {} & {} \\
{} & \multirow{-2}{*}{$\mathcal{O}({\epsilon}^{-3.5})$} & \multirow{-2}{*}{$\mathcal{O}({\epsilon}^{-2.5})$} &  \multirow{-2}{*}{-} \\
\rowcolor{gray!10} \multicolumn{1}{c}{} & {} & {} & {} \\
\rowcolor{gray!10} \multirow{-2}{*}{SimPO \citep{meng2024simpo}} & \multirow{-2}{*}{$\mathcal{O}(\frac{{\epsilon}^{-3.5}}{N})$} & \multirow{-2}{*}{$\mathcal{O}(\frac{{\epsilon}^{-2.5}}{N})$} & \multirow{-2}{*}{-} \\

{KTO \citep{ethayarajh2024model}} & {$\mathcal{O}({\epsilon}^{-3.5})$} & {$\mathcal{O}({\epsilon}^{-2.5})$} & {-} \\

\rowcolor{gray!10} {\textbf{MaPPO}} & {$\mathcal{O}({\epsilon}^{-3.5})$} & {$\mathcal{O}({\epsilon}^{-2.5})$} & {-} \\
\bottomrule[1.1pt]
\end{tabular}
\end{table}
\fi



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Preliminary \& Problem Setup}
\label{Sec:Problem_Setup}

\subsection{RL Tuning}

First, we introduce the general framework of Reinforcement Learning (RL). Consider the Markov decision process (MDP) as a tuple $( \mathcal{S}, \mathcal{A}, \mathcal{P}, \mathcal{R})$, where $\mathcal{S}$ is the state space, $\mathcal{A}$ is a finite action space, $\mathcal{P}:\mathcal{S}\times\mathcal{A}\times\mathcal{S}\rightarrow\mathbb{R}$ is a Markov kernel that determines transition probabilities, and $\mathcal{R}:\mathcal{S}\times\mathcal{A}\rightarrow\mathbb{R}$ is a reward function. 
At each time step $t$, the agent executes an action $\mathbf{y}_t \in\mathcal{A}$ from the current state $\mathbf{s}_t \in\mathcal{S}$, following a stochastic policy $\pi$, \textit{i.e.}, $\mathbf{y}_t \sim \pi(\cdot|\mathbf{s}_t)$. 
The corresponding reward is defined as $r_t$.

Following the conventional setting in LLMs, the policy $\pi_{\theta}$ represents the LLM with model parameters $\theta$. The action space $\mathcal{A}$ is set as the vocabulary. At step $t$, $\mathbf{s}_t=(\mathbf{x}, \mathbf{y}_{<t})$ is a cascade of the query $\mathbf{x}$ and the tokens $\mathbf{y}_{<t} = (\mathbf{y}_{1}, \cdots, \mathbf{y}_{t-1})$ that have been predicted, and $\mathbf{y}_t$ is the next token to be predicted. The transition kernel $\mathcal{P}$ is deterministic as $\mathbf{s}_{t+1} = (\mathbf{s}_t, \mathbf{y}_t)$. The complete answer $\mathbf{y}=(\mathbf{y}_{1}, \cdots,\mathbf{y}_{T})$ with length $|\mathbf{y}|=T$. The step reward $r_t = r(\mathbf{x}, \mathbf{y}_{\le t})$ can be obtained from a trained reward model.

After formalizing the LLM tuning as an RL problem, the goal of RL tuning~\citep{ouyang2022training} is to maximize the expectation of the cumulative reward $r \coloneqq r(\mathbf{x}, \mathbf{y})$  with a Kullback–Leibler (KL) constraint as follows
\begin{equation}
\label{eq:rl_target}
\begin{aligned}
    \max_{\pi_{\theta}} \mathop{\mathbb{E}}_{\mathbf{x}\sim\mathcal{D}, \mathbf{y}\sim\pi_{\theta}(\cdot|\mathbf{x})} \left[ r(\mathbf{x}, \mathbf{y}) \right] - \beta \mathbb{D}_{\rm KL} \left[ \pi_{\theta}(\cdot|\mathbf{x})||\pi_{\rm ref}(\cdot|\mathbf{x}) \right],
\end{aligned}
\end{equation}
where $\mathbb{D}_{\rm KL}(\cdot || \cdot)$ denotes the KL divergence, and $\beta$ is a constant weight. $\pi_{\rm ref}$ is a reference model, which is usually the initial policy model before tuning. This optimization problem can be solved by any RL algorithms, e.g., PPO \citep{schulman2017proximal} and GRPO \citep{shao2024deepseekmath}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Direct Preference Optimization}

In Direct Preference Optimization (DPO) \citep{dpo_neurips2023}, a closed-form expression of \eqref{eq:rl_target} is used, and a connection between policy $\pi$ and reward function $r$ is built as
\begin{equation}
\label{eq:r_pi_closed}
\begin{aligned}
    \pi( \mathbf{y} | \mathbf{x} ) ~=~& 
    \frac{1}{Z(\mathbf{x})} \pi_{\rm ref}( \mathbf{y} | \mathbf{x} ) \exp \big( \frac{1}{\beta} r(\mathbf{y}, \mathbf{x}) \big),
\end{aligned}
\end{equation}
where $Z(\mathbf{x})$ is a partition function to normalize the probability.

With a prompt $\mathbf{x}$, we sample two responses from the current policy model $\mathbf{y}_{1}, \mathbf{y}_{2} \sim\pi_{\theta}(\cdot|\mathbf{x})$. 
A human expert then demonstrates the preference and ranks the responses as $\mathbf{y}_{w}$ (win) and $\mathbf{y}_{l}$ (lose). 
After plugging in \eqref{eq:r_pi_closed} into the reward model training (MLE) loss function, the target of RL tuning becomes to minimize the loss function shown below
\begin{equation}
\label{eq:dpo_loss}
\begin{aligned}
    \mathcal{L}(\theta) ~=~& 
    \mathop{\mathbb{E}}_{( \mathbf{y}_{w}, \mathbf{y}_{l}, \mathbf{x})\sim\mathcal{D}} \Big[ -\log \sigma \Big( \beta\log \frac{\pi_{\theta}(\mathbf{y}_{w}|\mathbf{x})}{\pi_{\rm ref}(\mathbf{y}_{w}|\mathbf{x})} - \beta\log \frac{\pi_{\theta}(\mathbf{y}_{l}|\mathbf{x})}{\pi_{\rm ref}(\mathbf{y}_{l}|\mathbf{x})} \Big)\Big],
\end{aligned}
\end{equation}
where $\sigma (\cdot)$ is the logistic function. The training process can be done using mini-batch gradient descent and the variants, e.g., AdamW \citep{loshchilov2018decoupled}. Notably, the derivation on reward model training is based on MLE, which oversimplifies the process as a binary classification problem. As a result, minimizing \eqref{eq:dpo_loss} is nothing but increasing the gap between the output probability of $\mathbf{y}_{w}$ and $\mathbf{y}_{l}$.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Current issues with MLE}

The learning process is to estimate the parameters $\theta$ via maximum likelihood, which is to maximize the gap of the output probability between the winning response $\pi_{\theta}(\mathbf{y}_{w}|\mathbf{x})$ and the losing response $\pi_{\theta}(\mathbf{y}_{l}|\mathbf{x})$.

Despite its computational efficiency and simplicity, the MLE formulation introduces a critical limitation: It focuses solely on relative probabilities within each preference pair, while ignoring the absolute magnitude of confidence in the responses. Shown as Figure~\ref{fig:compare_MLE_MAP}, training encourages simultaneous downscaling of both $\pi_{\theta}(\mathbf{y}_{w}|\mathbf{x})$ and $\pi_{\theta}(\mathbf{y}_{l}|\mathbf{x})$, to enlarge the preference gap. This undesired tendency can lead to over-penalization of both responses, especially in near-tie cases, thereby reducing output confidence and harming policy calibration~\citep{ren2024learning}.

Such issues become particularly problematic as models approach human-level performance, where both the winning and losing responses may be of high quality. For example, consider a preference pair where both $\mathbf{y}_{w}$ and $\mathbf{y}_{l}$ are grammatically correct, contextually relevant, and factually accurate, with the only preference driven by stylistic nuances. In this case, the MLE objective may still enforce a large probability gap by downscaling both log-likelihoods. This inadvertently shifts the probability mass away from the high-quality response space, introducing unnecessary uncertainty into the policy, and can lead to erratic or unstable generation in downstream usage.

\begin{figure}[!ht]
\vspace{-3mm}
\begin{tcolorbox}[title=Prompt~$\mathbf{x}$, fonttitle=\bfseries, boxrule=0.5mm]
A printer prints 17 pages per minute. How many minutes will it take to print 200 pages? Express your answer to the nearest whole number.
\end{tcolorbox}
\begin{tcolorbox}[colback=green!5, colframe=black!60!green!45, title={\textbf{Response}~$\mathbf{y}_{w}$, $r=0.95$}, fonttitle=\bfseries, boxrule=0.5mm]
To find out how many minutes it will take to print 200 pages, we need to divide the total number of pages by the number of pages the printer can print per minute.
So we divide 200 by 17: $\frac{200}{17} \approx 11.76$.
But since we want the nearest whole number, we need to round it up. That means it will take $\boxed{12}$ minutes to print 200 pages. The answer is: $\boxed{12}$
\end{tcolorbox}
\begin{tcolorbox}[colback=red!5, colframe=black!60!red!45, title={\textbf{Response}~$\mathbf{y}_{l}$, $r=0.91$}, fonttitle=\bfseries, boxrule=0.5mm]
To find out how many minutes it will take to print 200 pages at a rate of 17 pages per minute, divide: $\frac{200}{17} \approx 11.76$.
Rounding 11.76 to the nearest whole number gives: $12$.
So it will take $\boxed{12}$ minutes to print 200 pages. The answer is: $\boxed{12}$
\end{tcolorbox}
\vspace{-4mm}
\caption{An example of $(\mathbf{x}, \mathbf{y}_{w}, \mathbf{y}_{l})$ pair. Both responses $\mathbf{y}_{w}$ and $\mathbf{y}_{l}$ have good quality as they achieve high rewards, where $r(\mathbf{x}, \mathbf{y}_{w}) = 0.95$, $r(\mathbf{x}, \mathbf{y}_{l}) = 0.91$, and $r \in [0,1]$.}
\label{fig:prompt_example}
\end{figure}

\begin{table}[!ht]
\centering
\caption{Comparison of log-probabilities for responses $\mathbf{y}_w$ and $\mathbf{y}_l$ in PO methods.}
\label{table:logp_gap_comparison}
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{logp($\mathbf{y}_w$)} & \textbf{logp($\mathbf{y}_l$)} & \textbf{logp($\mathbf{y}_w$) - logp($\mathbf{y}_l$)} \\
\midrule
IT         & $-14.3$    & $-43.4$    & $+29.1$ \\
DPO        & \textcolor{red}{$-121.5$}   & $-443.2$   & $+321.7$ \\
MaPPO      & \textcolor{black!50!green!80}{$-10.4$}    & $-321.1$   & $+310.7$ \\
\bottomrule
\end{tabular}
\end{table}

In Figure \ref{fig:prompt_example}, we show an example of the prompt and response pair $(\mathbf{x}, \mathbf{y}_{w}, \mathbf{y}_{l})$.  
Given the prompt $\mathbf{x}$, both $\mathbf{y}_{w}$ and $\mathbf{y}_{l}$ have correct answers, while in slightly different expressions. 
Both $\mathbf{y}_{w}$ and $\mathbf{y}_{l}$ have high rewards, which reflect the high qualities.
However, in MLE and its derived DPO, the learning objective is nothing but to increase the gap between $\mathbf{y}_{w}$ and $\mathbf{y}_{l}$, regardless of the fact that both of them have high qualities with correct answers, and their qualities match each other. 
We also list an example with long responses in Appendix \ref{app:Supplementary_Examples}.
As shown in Table \ref{table:logp_gap_comparison}, after DPO training, the log output probability of $\mathbf{y}_{w}$ decreases from $-14.3$ to $-121.5$, and $\mathbf{y}_{l}$ decreases from $-43.4$ to $-443.2$. Although the gap indeed increases from $29.1$ to $321.7$, it violates the principal goal: Increase the output probability of the high-quality responses.

These issues highlight the need for a more principled formulation that preserves relative preferences while incorporating global calibration and prior reward knowledge. In the next section, we introduce our Maximum-a-Posteriori (MaP) framework that addresses these shortcomings in a unified and efficient manner.

\begin{figure}[!htbp]
\vspace{-4mm}
    \centering
    \includegraphics[width=\linewidth]{figures/compare_MLE_MAP.pdf}
\vspace{-4mm}
    \caption{Under the standard MLE-based DPO (left), empirical studies~\citep{pal2024smaug, rafailov2024r, tajwar2024preference, ren2024learning} demonstrated that training tends to simultaneously downscale (with different magnitudes) both the chosen and rejected responses to increase their gap. Our MaP-based method (right) mitigates this harmful tendency by re-weighting the rejected response based on prior knowledge. Here, the x-axis denotes the initial model $\theta_0$ and a potentially harmful model $\theta_k$ that may arise during training, while the y-axis shows the log-likelihood of a fixed preference pair under different policies.}
    \label{fig:compare_MLE_MAP}
\end{figure}


% \subsection{SFT}

% In supervised learning, with a prompt $\mathbf{x}$, a human expert demonstrates an answer $\mathbf{y}^{+}$, which is taken as the true answer. The learning process is to estimate the parameters $\theta$ via maximum likelihood, which is equivalent to minimizing the cross entropy loss between the output $\pi_{\theta}(\cdot|\mathbf{x})$ and the true label. We denote the cross entropy loss as $H\left( P^{+}(\cdot |\mathbf{x}), \pi_{\theta}(\cdot |\mathbf{x}) \right) \coloneqq -\sum_{\mathbf{y}} P^{+}(\mathbf{y} |\mathbf{x}) \log \pi_{\theta}(\mathbf{y}|\mathbf{x})$, where $P^{+}(\cdot |\mathbf{x})$ is the correct distribution. Specifically, $P^{+}(\mathbf{y} |\mathbf{x}) = \mathds{1}_{\mathbf{y} = \mathbf{y}^{+}}$.
% \begin{equation}
% \label{eq:ce_loss}
% \begin{aligned}
%     \mathcal{L}_{+}(\theta) ~\coloneqq~& \mathop{\mathbb{E}}_{(\mathbf{x}, \mathbf{y}^{+})\sim\mathcal{D}} \left[ \ell_{+} \left(\theta; (\mathbf{x}, \mathbf{y}^{+}) \right) \right] \\
%     =& \mathop{\mathbb{E}}_{(\mathbf{x}, \mathbf{y}^{+})\sim\mathcal{D}} \left[ H\left( P^{+}(\cdot |\mathbf{x}), \pi_{\theta}(\cdot |\mathbf{x}) \right) \right] = \mathop{\mathbb{E}}_{(\mathbf{x}, \mathbf{y}_{\checkmark})\sim\mathcal{D}} \left[ -\log \pi_{\theta}(\mathbf{y}_{\checkmark}|\mathbf{x}) \right].
% \end{aligned}
% \end{equation}

% With negative result $\mathbf{y}^{-}$, the undesired distribution is $P^{-}(\mathbf{y} |\mathbf{x}) = \mathds{1}_{\mathbf{y} = \mathbf{y}^{-}}$. The target can be further changed to
% \begin{equation}
% \label{eq:ce_loss_neg}
% \begin{aligned}
%     \mathcal{L}_{\pm}(\theta) ~\coloneqq~& \mathop{\mathbb{E}}_{(\mathbf{x}, \mathbf{y}^{+}, \mathbf{y}^{-})\sim\mathcal{D}} \Big[ \ell_{\pm} \left(\theta; (\mathbf{x}, \mathbf{y}^{+}, \mathbf{y}^{-}) \right) \Big] \\ 
%     ~=~& \mathop{\mathbb{E}}_{(\mathbf{x}, \mathbf{y}^{+}, \mathbf{y}^{-})\sim\mathcal{D}} \left[ H\left( P^{+}(\cdot |\mathbf{x}), \pi_{\theta}(\cdot |\mathbf{x}) \right) - \alpha H\left( P^{-}(\cdot |\mathbf{x}), \pi_{\theta}(\cdot |\mathbf{x}) \right) \right] \\
%     ~=~& \mathop{\mathbb{E}}_{(\mathbf{x}, \mathbf{y}_{\checkmark}, \mathbf{y}_{\times})\sim\mathcal{D}} \left[ -\log \pi_{\theta}(\mathbf{y}_{\checkmark}|\mathbf{x}) + {\alpha} \log\pi_{\theta}(\mathbf{y}_{\times}|\mathbf{x}) \right], \\
%     ~=~& \mathop{\mathbb{E}}_{(\mathbf{x}, \mathbf{y}^{+}, \mathbf{y}^{-})\sim\mathcal{D}} \left[ -\log \frac{\pi_{\theta}(\mathbf{y}^{+}|\mathbf{x})}{\pi_{\theta}^{\alpha}(\mathbf{y}^{-}|\mathbf{x})} \right],
% \end{aligned}
% \end{equation}
% where $\alpha$ is the weight constant. $\alpha=1$ if they have equal weights.






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{MaPPO Design}
\label{Sec:mappo}

\subsection{MaPPO Loss}
\label{Sec:mappo_loss}

In this subsection, we start the derivation step by step from the first principle. 

With a prompt $\mathbf{x}$ and responses $(\mathbf{y}_{1}, \mathbf{y}_{2})$, an oracle gives its preference on the responses as $(\mathbf{y}_{w}, \mathbf{y}_{l})$. The Bradley-Terry (BT) model \citep{bradley1952rank} builds the connection between the rewards and the preference probability as follows:
\begin{equation}
\label{eq:bt_model}
\begin{aligned}
    p(\mathbf{y}_{w} \succ \mathbf{y}_{l} | \mathbf{x}) ~=~ \frac{ \exp( r(\mathbf{y}_{w}, \mathbf{x}) ) }{\exp( r(\mathbf{y}_{w}, \mathbf{x}) ) + \exp( r(\mathbf{y}_{l}, \mathbf{x}) )}
    ~=~ \frac{1}{1 + \exp( r(\mathbf{y}_{l}, \mathbf{x}) - r(\mathbf{y}_{w}, \mathbf{x}) )}.
\end{aligned}
\end{equation}
The preference dataset have $N$ samples denoted as $\mathcal{D} = \{\mathbf{y}_{w}^{i}, \mathbf{y}_{l}^{i}, \mathbf{x}^{i}\}_{i=1}^{N}$. We can parametrize a reward model with model parameters $\phi$ as $r_{\phi}(\mathbf{y}, \mathbf{x})$. Given $\mathbf{x}$, assume we have prior knowledge of rewards as $r_{w}$ and $r_{l} \in [-1,0]$. This can be obtained from an oracle, \textit{e.g.}, a pre-trained reward model. To incorporate the prior knowledge of rewards, we need to use the gap $\Delta_{r} = r_{w} - r_{l}$ as suggested in \eqref{eq:bt_model}. To keep the softmax form in the BT model, we can construct the prior probability as follows
\begin{equation}
\label{eq:prior_prob}
\begin{aligned}
p(r_{\phi}) ~=~ \frac{ \exp( r_{\phi}(\mathbf{y}_{w}, \mathbf{x}) ) + \exp( \Delta_{r} r_{\phi}(\mathbf{y}_{l}, \mathbf{x}) )}{ \exp( r_{\phi}(\mathbf{y}_{w}, \mathbf{x}) ) + \exp( r_{\phi}(\mathbf{y}_{l}, \mathbf{x}) )}.
\end{aligned}
\end{equation}

We use the reward gap $\Delta_{r}$ on the softmax probability to make the probability always greater than $0$ and smaller than $1$. 
% We show the proof in Appendix \ref{app:proof_prob_nike}. 
Notably, this form is not unique, and other forms are also acceptable if they satisfy the properties of the probability function. We further discuss the prior function in Appendix \ref{app:Prior_Function}.

The MaP loss is the combination of the MLE loss and the prior knowledge loss as follows
\begin{equation}
\label{eq:map_mle_loss}
\begin{aligned}
    \mathcal{L}_{\rm MaP}(r_{\phi}) ~=~& \mathcal{L}_{\rm MLE}(r_{\phi}) + \mathcal{L}_{\rm p}(r_{\phi}) \\
    ~=~& \mathop{\mathbb{E}}_{( \mathbf{y}_{w}, \mathbf{y}_{l}, \mathbf{x})\sim\mathcal{D}} \Big[ -\log \sigma \Big( r_{\phi}(\mathbf{y}_{w}, \mathbf{x}) - r_{\phi}(\mathbf{y}_{l}, \mathbf{x})\Big) - \log p(r_{\phi})\Big] \\
    ~=~& \mathop{\mathbb{E}}_{( \mathbf{y}_{w}, \mathbf{y}_{l}, \mathbf{x})\sim\mathcal{D}} \Big[ -\log \sigma \Big(  r_{\phi}(\mathbf{y}_{w}, \mathbf{x}) - \Delta_{r} r_{\phi}(\mathbf{y}_{l}, \mathbf{x})\Big)\Big].
\end{aligned}
\end{equation}

% Note that the function $\log \sigma (\cdot)$ is monotonic. Thus, we can multiply a constant inside, which does not change the optimality but only the learning rate. To make the loss function more concise, we modify it as 
% \begin{equation}
% \label{eq:map_r_loss}
% \begin{aligned}
%     \mathcal{L}_{\rm MaP}(r_{\phi}) ~=~& 
%     \mathop{\mathbb{E}}_{( \mathbf{y}_{w}, \mathbf{y}_{l}, \mathbf{x})\sim\mathcal{D}} \Big[ -\log \sigma \Big( r_{\phi}(\mathbf{y}_{w}, \mathbf{x}) - \Delta_{r}^{2} r_{\phi}(\mathbf{y}_{l}, \mathbf{x})\Big)\Big].
% \end{aligned}
% \end{equation}

As proved in previous works \citep{dpo_neurips2023, go2023aligning, korbak2022on}, given a reward function $r(\mathbf{y}, \mathbf{x})$, we have a closed-form expression of the policy $\pi$ as
\begin{equation}
\label{eq:r_pi}
\begin{aligned}
    \pi( \mathbf{y} | \mathbf{x} ) ~=~& 
    \frac{1}{Z(\mathbf{x})} \pi_{\rm ref}( \mathbf{y} | \mathbf{x} ) \exp \big( \frac{1}{\beta} r(\mathbf{y}, \mathbf{x}) \big),
\end{aligned}
\end{equation}
where $Z(\mathbf{x})$ is a partition function. With a parametrized policy $\pi_{\theta}$, we can plug this result into the loss function \eqref{eq:map_mle_loss}, and get the MaPPO loss
\begin{equation}
\label{eq:mappo_loss}
\begin{aligned}
    \mathcal{L}_{\rm MaP}(\theta) ~=~& 
    \mathop{\mathbb{E}}_{( \mathbf{y}_{w}, \mathbf{y}_{l}, \mathbf{x})\sim\mathcal{D}} \Big[ -\log \sigma \Big( \beta\log \frac{\pi_{\theta}(\mathbf{y}_{w}|\mathbf{x})}{\pi_{\rm ref}(\mathbf{y}_{w}|\mathbf{x})} - \Delta_{r} \beta\log \frac{\pi_{\theta}(\mathbf{y}_{l}|\mathbf{x})}{\pi_{\rm ref}(\mathbf{y}_{l}|\mathbf{x})} \Big)\Big].
\end{aligned}
\end{equation}

With the MaP estimation, we achieve a clean result compared to the MLE estimation in DPO with a calibration term $\Delta_{r} \in [0, 1]$ from the prior knowledge.

\paragraph{Remark.}
In our MaPPO method, \textbf{no} additional hyperparameter is introduced compared to the original DPO method. Thus, MaPPO offers a clean and easily pluggable solution, and no extra hyperparameter tuning is needed.


\subsection{Analysis of MaPPO}

In this subsection, we analyze the connection with MaPPO and DPO.

% \paragraph{Connection with SFT.} 

% % which is equivalent to the SFT loss function, and $\mathbf{y}_{w}$ is the supervised target. The reason is that the function $\log \sigma (\cdot)$ is monotonic. Thus, the optimal solution is equal to that from the loss function below
% First, in the SFT loss function, the optimal solution is equal to that from the loss function below
% \begin{equation}
% \label{eq:mappo_loss_sft}
% \begin{aligned}
%     \mathcal{L}(\theta) ~=~& 
%     \mathop{\mathbb{E}}_{( \mathbf{y}_{w}, \mathbf{y}_{l}, \mathbf{x})\sim\mathcal{D}} \Big[ -\log \frac{\pi_{\theta}(\mathbf{y}_{w}|\mathbf{x})}{\pi_{\rm ref}(\mathbf{y}_{w}|\mathbf{x})} \Big],
% \end{aligned}
% \end{equation}
% where $\mathbf{y}_{w}$ is the supervised target.

% The gradient is
% \begin{equation}
% \label{eq:mappo_loss_sft_grad}
% \begin{aligned}
%     \mathop{\mathbb{E}}_{( \mathbf{y}_{w}, \mathbf{y}_{l}, \mathbf{x})\sim\mathcal{D}} \Big[ - \nabla \log \frac{\pi_{\theta}(\mathbf{y}_{w}|\mathbf{x})}{\pi_{\rm ref}(\mathbf{y}_{w}|\mathbf{x})} \Big] ~=~
%     \mathop{\mathbb{E}}_{( \mathbf{y}_{w}, \mathbf{y}_{l}, \mathbf{x})\sim\mathcal{D}} \Big[ -\nabla \log {\pi_{\theta}(\mathbf{y}_{w}|\mathbf{x})} \Big]  ~=~ \nabla \mathcal{L}_{\rm SFT}(\theta).
% \end{aligned}
% \end{equation}

% In \eqref{eq:mappo_loss}, when $r_{w}=r_{l}~({i.e.},~\Delta_{r}=0)$, the loss function becomes
% \begin{equation}
% \label{eq:mappo_loss_0}
% \begin{aligned}
%     \mathcal{L}(\theta) ~=~& 
%     \mathop{\mathbb{E}}_{( \mathbf{y}_{w}, \mathbf{y}_{l}, \mathbf{x})\sim\mathcal{D}} \Big[ -\log \sigma \Big( \beta\log \frac{\pi_{\theta}(\mathbf{y}_{w}|\mathbf{x})}{\pi_{\rm ref}(\mathbf{y}_{w}|\mathbf{x})} \Big)\Big].
% \end{aligned}
% \end{equation}
% As the function $\log \sigma (\cdot)$ is monotonic, its stochastic gradient has the same direction as the SFT loss function, and only differs in learning steps. Notably, with online response data collection ($\mathbf{y}_{w}$ is generated from the current policy model $\pi_{\theta}$), this is also known as the Reject Sampling (RS) method \citep{dong2023raft}.


\paragraph{Connection with DPO.} In \eqref{eq:mappo_loss}, when $r_{w}=0$ and $r_{l}=-1$, we have $\Delta_{r}=1$. The loss function becomes
\begin{equation}
\label{eq:mappo_loss_1}
\begin{aligned}
    \mathcal{L}(\theta) ~=~& 
    \mathop{\mathbb{E}}_{( \mathbf{y}_{w}, \mathbf{y}_{l}, \mathbf{x})\sim\mathcal{D}} \Big[ -\log \sigma \Big( \beta\log \frac{\pi_{\theta}(\mathbf{y}_{w}|\mathbf{x})}{\pi_{\rm ref}(\mathbf{y}_{w}|\mathbf{x})} - \beta\log \frac{\pi_{\theta}(\mathbf{y}_{l}|\mathbf{x})}{\pi_{\rm ref}(\mathbf{y}_{l}|\mathbf{x})} \Big)\Big],
\end{aligned}
\end{equation}
which degenerates to the DPO loss function in \eqref{eq:dpo_loss}. 

% Overall, both DPO and SFT loss functions (I-DPO and RS in the online setting) can be taken as \emph{special cases} of MaPPO. In this sense, MaPPO can be taken as a dynamic weighted mechanism, where the weight depends on the relative quality (rewards) of the winning response $\mathbf{y}_{w}$ and the losing response $\mathbf{y}_{l}$.
Overall, DPO loss function can be taken as \emph{special cases} of MaPPO. In this sense, MaPPO can be taken as a dynamic weighted mechanism, where the weight depends on the relative quality (rewards) of the winning response $\mathbf{y}_{w}$ and the losing response $\mathbf{y}_{l}$.

\paragraph{Gradient Dynamics Analysis.} To analyze the update of MaPPO, the gradient of \eqref{eq:mappo_loss} is
\begin{equation}
\label{eq:mappo_grad}
\begin{aligned}
    \nabla \mathcal{L}_{\rm MaP}(\theta) ~=~&
    \mathop{\mathbb{E}}_{( \mathbf{y}_{w}, \mathbf{y}_{l}, \mathbf{x})\sim\mathcal{D}} \Big[ -\beta (1-\sigma(u)) \Big( \nabla \log {\pi_{\theta}(\mathbf{y}_{w}|\mathbf{x})} - \Delta_{r} \nabla \log {\pi_{\theta}(\mathbf{y}_{l}|\mathbf{x})} \Big)\Big],
\end{aligned}
\end{equation}
where $u = \beta \big( \log \frac{\pi_{\theta}(\mathbf{y}_{w}|\mathbf{x})}{\pi_{\rm ref}(\mathbf{y}_{w}|\mathbf{x})} - \Delta_{r} \log \frac{\pi_{\theta}(\mathbf{y}_{l}|\mathbf{x})}{\pi_{\rm ref}(\mathbf{y}_{l}|\mathbf{x})} \big)$ serves as a confidence measure of preference separation. 
$1-\sigma(u)$ down-weights the gradient when the model is already confident in distinguishing $\mathbf{y}_{w}$ and $\mathbf{y}_{l}$. 
$\Delta_{r}$ directly scales the contribution of the losing sample $\mathbf{y}_{l}$, modulating the penalization. 
The gradient norm of MaPPO is upper-bounded compared to DPO, leading to less aggressive updates and more stable policy calibration. 
We provide a more detailed theoretical analysis, including the stationary convergence analysis in Appendix \ref{app:theo_converge} and Lipschitz stability analysis in Appendix \ref{app:Lipschitz}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Online MaPPO}
\label{sec:online_mappo}

Beyond the offline setting, our MaPPO method can be directly used in the online or iterative settings. As shown in Algorithm \ref{algo:depo}, we describe the online version of MaPPO. In online MaPPO, one key difference is that the responses $\{\mathbf{y}\}$ are generated online from the current policy $\pi_{\theta}$ instead of the initial policy $\pi_{\theta_{0}}$ in the offline setting.


\begin{algorithm}[!ht]
\caption{Online MaPPO}
\label{algo:depo}
\begin{algorithmic}[1] %[1] enables line numbers
\REQUIRE {Prompt data set $\mathcal{D}$; Number of iterations $K$; Initial policy model ${\theta_{0}}$.}
\STATE {\textbf{for} $k = 0, \cdots, K-1$ \textbf{do}}
\STATE {~~~~~~~~Sample a prompt $\mathbf{x} \sim\mathcal{D}$.}
\STATE {~~~~~~~~Sample responses from the current policy $\mathbf{y}_{w}, \mathbf{y}_{l} \sim \pi_{\theta_{k}}(\cdot | \mathbf{x})$.}
\STATE {~~~~~~~~Get corresponding rewards $r_{w} \leftarrow r(\mathbf{y}_{w}, \mathbf{x})$ and $r_{l} \leftarrow r(\mathbf{y}_{l}, \mathbf{x})$.}
\STATE {~~~~~~~~$\Delta_{r} \leftarrow r(\mathbf{y}_{w}, \mathbf{x}) - r(\mathbf{y}_{l}, \mathbf{x})$}
\STATE {~~~~~~~~Compute $\mathcal{L}(\theta_{k})$ according to \eqref{eq:mappo_loss}.}
\STATE {~~~~~~~~$\theta_{k+1} \leftarrow \theta_{k} - \eta \nabla \mathcal{L}(\theta_{k})$~~~~\# Or other optimizer, e.g., AdamW.}
\STATE {\textbf{end for}}
\ENSURE
{${\theta_{K}}$}
\end{algorithmic}
\end{algorithm}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/i_mappo.pdf}
    \caption{Illustration of the iterative MaPPO pipeline in each iteration $k$.}
    \label{fig:i_mappo}
\end{figure}

In practice, considering training efficiency, online PO can be implemented in an iterative way, known as I-DPO \citep{dong2024rlhf}. 
In Figure \ref{fig:i_mappo}, we illustrate the iterative MaPPO pipeline.
With a prompt set $\mathcal{D}$, we can equally divide $\mathcal{D}$ into $K$ subsets as $\mathcal{D}_{1} \cdots \mathcal{D}_{K}$. 
In the $k$-th iteration, we first freeze the current policy model $\pi_{\theta}$, and then get responses $(\mathbf{y}_{1}, \mathbf{y}_{2})$ from the policy according to the prompt set $\mathcal{D}_{k}$. 
We then use a reward model to get the responses' corresponding rewards and collect $(\mathbf{y}_{w}, \mathbf{y}_{l})$ pairs, which reflect the preference. 
After response collection on $\mathcal{D}_{k}$, we conduct the MaPPO training process using \eqref{eq:mappo_loss} on the subset $\mathcal{D}_{k}$. 
After training on the prompt subset, we repeat the process in the next iteration $k+1$ until we finish all $K$ training iterations.

\paragraph{Remark.}
A reward model (or rule-based verifier) is necessary for all online methods, including online DPO (iterative DPO) \citep{dong2024rlhf} and reject sampling \citep{dong2023raft}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Adaptation to Other PO Methods}
\label{sec:adapt_other_po}

We have shown MaPPO in the offline and online DPO settings. As this Maximum a Posteriori (MaP) method is generally suitable for all DPO variants, we show how MaPPO modifies other DPO variants in this subsection.

Simply replace the MLE part in preference optimization with MaP, and follow the same derivation in Section \ref{Sec:mappo_loss}. Most DPO variants, as long as MLE is used in the original methods, can be modified with MaPPO as a plugin. We show some widely adopted methods as examples here, including SimPO, IPO, and CPO. 

First, in SimPO \citep{meng2024simpo}, with the length control penalty, the loss function is given as
\begin{equation}
\label{eq:simpo}
\begin{aligned}
    \mathcal{L}_{\rm SimPO}(\theta) ~=~& 
    \mathop{\mathbb{E}}_{( \mathbf{y}_{w}, \mathbf{y}_{l}, \mathbf{x})\sim\mathcal{D}} \Big[ -\log \sigma \Big( \frac{\beta}{|\mathbf{y}_{w}|} \log {\pi_{\theta}(\mathbf{y}_{w}|\mathbf{x})} - \frac{\beta}{|\mathbf{y}_{l}|} \log {\pi_{\theta}(\mathbf{y}_{l}|\mathbf{x})} - \gamma \Big)\Big],
\end{aligned}
\end{equation}
where $\gamma$ is a constant hyperparameter, $|\mathbf{y}_{w}|$ and $|\mathbf{y}_{l}|$ denote the length of $\mathbf{y}_{w}$ and $\mathbf{y}_{l}$, respectively.

With the MaPPO plugin, the loss function is modified as 
\begin{equation}
\label{eq:simpo_mappo}
\begin{aligned}
    \mathcal{L}_{\rm SimPO+}(\theta) ~=~& 
    \mathop{\mathbb{E}}_{( \mathbf{y}_{w}, \mathbf{y}_{l}, \mathbf{x})\sim\mathcal{D}} \Big[ -\log \sigma \Big( \frac{\beta}{|\mathbf{y}_{w}|} \log {\pi_{\theta}(\mathbf{y}_{w}|\mathbf{x})} - \Delta_{r} \frac{\beta}{|\mathbf{y}_{l}|} \log {\pi_{\theta}(\mathbf{y}_{l}|\mathbf{x})} - \gamma \Big)\Big].
\end{aligned}
\end{equation}

In IPO \citep{azar2024general}, the original loss function is
\begin{equation}
\label{eq:IPO}
\begin{aligned}
    \mathcal{L}_{\rm IPO}(\theta) ~=~& 
    \mathop{\mathbb{E}}_{( \mathbf{y}_{w}, \mathbf{y}_{l}, \mathbf{x})\sim\mathcal{D}} \Big[ \Big( \log \frac{\pi_{\theta}(\mathbf{y}_{w}|\mathbf{x})}{\pi_{\rm ref}(\mathbf{y}_{w}|\mathbf{x})} - \log \frac{\pi_{\theta}(\mathbf{y}_{l}|\mathbf{x})}{\pi_{\rm ref}(\mathbf{y}_{l}|\mathbf{x})} - \frac{1}{2\beta} \Big)^{2} \Big].
\end{aligned}
\end{equation}
With the MaPPO plugin, the loss function is modified as 
\begin{equation}
\label{eq:IPO_mappo}
\begin{aligned}
    \mathcal{L}_{\rm IPO+}(\theta) ~=~& 
    \mathop{\mathbb{E}}_{( \mathbf{y}_{w}, \mathbf{y}_{l}, \mathbf{x})\sim\mathcal{D}} \Big[ \Big( \log \frac{\pi_{\theta}(\mathbf{y}_{w}|\mathbf{x})}{\pi_{\rm ref}(\mathbf{y}_{w}|\mathbf{x})} - \Delta_{r} \log \frac{\pi_{\theta}(\mathbf{y}_{l}|\mathbf{x})}{\pi_{\rm ref}(\mathbf{y}_{l}|\mathbf{x})} - \frac{1}{2\beta} \Big)^{2} \Big].
\end{aligned}
\end{equation}

In CPO \citep{xu2024contrastive}, the original loss is 
\begin{equation}
\label{eq:cpo}
\begin{aligned}
    \mathcal{L}_{\rm CPO}(\theta) ~=~& 
    \mathop{\mathbb{E}}_{( \mathbf{y}_{w}, \mathbf{y}_{l}, \mathbf{x})\sim\mathcal{D}} \Big[ -\log \sigma \Big( \beta \log {\pi_{\theta}(\mathbf{y}_{w}|\mathbf{x})} - \beta \log {\pi_{\theta}(\mathbf{y}_{l}|\mathbf{x})} \Big) - \lambda \log {\pi_{\theta}(\mathbf{y}_{w}|\mathbf{x})} \Big],
\end{aligned}
\end{equation}
where $\lambda$ is a constant hyperparameter.

With the MaPPO plugin, the CPO loss is modified as 
\begin{equation}
\label{eq:CPO_mappo}
\begin{aligned}
    \mathcal{L}_{\rm CPO+}(\theta) ~=~& 
    \mathop{\mathbb{E}}_{( \mathbf{y}_{w}, \mathbf{y}_{l}, \mathbf{x})\sim\mathcal{D}} \Big[ -\log \sigma \Big( \beta \log {\pi_{\theta}(\mathbf{y}_{w}|\mathbf{x})} - \beta \Delta_{r} \log {\pi_{\theta}(\mathbf{y}_{l}|\mathbf{x})} \Big) - \lambda \log {\pi_{\theta}(\mathbf{y}_{w}|\mathbf{x})} \Big].
\end{aligned}
\end{equation}

To verify the effectiveness, we show the experimental results with the improvement of these DPO variants in Section \ref{sec:adapt}.

\paragraph{Remark.}
With our MaPPO plugin, \textbf{no} additional hyperparameter is introduced in all DPO variants.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}
\label{Sec:Experiments}

In this section, we empirically verify the effectiveness of our MaPPO methods.

\subsection{Setup}
\label{sec:Experiments_setup}

\paragraph{Pipeline Settings.}
We follow the RLHF framework in \cite{dong2024rlhf}. 
Instead of costly human annotations, we employ off-the-shelf reward models to generate the preferences. We use the public pre-trained BT reward model\footnote{https://huggingface.co/sfairXC/FsfairX-LLaMA3-RM-v0.1} as the prior knowledge. For the response selection, we follow the rejection sampling strategy suggested by \cite{liustatistical, gulcehre2023reinforced}. 
For each prompt, we generate $n = 8$ responses and use the best-of-8 as $\mathbf{y}_{w}$ and the worst-of-8 as $\mathbf{y}_{l}$. We provide hyperparameter details and computing resources in Appendix \ref{mappo:sec:app_exp_setting}.

\paragraph{Dataset.}
We use the prompt set in \cite{dong2024rlhf}. In the offline setting, we generate responses from the initial model with the whole prompt set. In the online (iterative) setting, we separate the prompt set into three subsets of the same size. 
The learning process lasts for $K = 3$ iterations. 
In each iteration, we sample responses from our current policy with one prompt subset, and use preference signals on these responses to improve our policy.

\paragraph{Models.}
To show the scalability of our methods, we choose models in two dimensions: (1) \textit{Model sizes}: Qwen2.5-1.5B-Instruct, Qwen2.5-3B-Instruct, and Qwen2.5-7B-Instruct. (2) \textit{Model series}: Qwen2.5-7B-Instruct, Mistral-7B-Instruct-v0.3, and Llama-3-8B-Instruct in our experiments.


\paragraph{Evaluation.}
We evaluate the model performance on three widely used benchmarks: MT-Bench \citep{zheng2023judging},
AlpacaEval 2.0 \citep{li2023alpacaeval}, and Arena-Hard v0.1 \citep{li2024live}. MT-Bench contains $80$ questions from $8$ categories, with answers rated by GPT-4 on a scale of $1-10$. Arena-Hard v0.1 contains $500$ technical problem-solving questions, and the answers are compared to reference responses from the baseline model GPT-4-0314. We report the win rate (WR) in percentage as judged by GPT-4 Turbo (Preview-1106). AlpacaEval 2.0 includes $805$ questions from five datasets, with the judge model GPT-4 Turbo (Preview-1106) comparing the answers to reference responses from itself. We report the length-controlled (LC) WR as suggested in \cite{dubois2024lengthcontrolled}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Main Results}

Our main results on three standard benchmarks, introduced in Section \ref{sec:Experiments_setup}, are shown in Table \ref{table:Evaluation}. 
For the alignment methods, we show the evaluation results of Instruction Tuning (IT), the original offline setting~\citep{dpo_neurips2023} (DPO), and the online setting~\citep{dong2024rlhf} (I-DPO) as described in Section \ref{sec:online_mappo}. 
For DPO and I-DPO, we show their improvements that incorporate the MaPPO design (+MaPPO). 

For Llama-3-8B-Instruct, Mistral-7B-Instruct, and Qwen2.5-7B-Instruct models, the performances are significantly improved with MaPPO on AlpacaEval 2.0 and Arena-Hard in both the offline setting (DPO) and the online setting (I-DPO). 
It reflects the effectiveness of MaPPO on different model series in both online and offline settings. 
On the MT-Bench, the performances are slightly improved on Qwen2.5-7B-Instruct and Llama-3-8B-Instruct, because the base models have already achieved very good results on this benchmark, which has limitations to reflect the effective improvement. 
The improvement on MT-Bench becomes much more significant on models with mediocre base or DPO performances, \textit{e.g.}, Mistral-7B-Instruct and Qwen2.5-1.5B-Instruct. 
In one model series, the larger models achieve higher overall scores in both base performances and after online \& offline alignment tuning, suggesting that scaling up model size enhances alignment capability as expected. 
With MaPPO, the improvement is consistent in scale with different model sizes in both online and offline settings, and the alignment can make smaller models outperform larger base models.

\begin{table}[!ht]
\vspace{-4mm}
\caption{Main evaluation results on three standard benchmarks. $\uparrow$ indicates the higher the better.}
\centering
 % \small
\label{table:Evaluation}
\begin{tabular}{l|l|lll}
\toprule[1.1pt]
% \hline
{Model} & {Method} & {AlpacaEval 2.0 $\uparrow$} & {Arena-Hard $\uparrow$} & {MT-Bench $\uparrow$} \\
\midrule[1.1pt]
\multirow{5}{*}{Qwen2.5-1.5B-Instruct} & {IT} & {11.10} &{5.0}&{7.06} \\
\cline{2-5}
{ } & {DPO} & {$18.71$} &{$11.6$}&{$7.29$} \\
{ } & {+\textbf{MaPPO}} & {$\mathbf{19.35}$ $\textcolor{ForestGreen}{+0.64}$} & {$\mathbf{15.3}$ $\textcolor{ForestGreen}{+3.7}$} & {$\mathbf{7.57}$ $\textcolor{ForestGreen}{+0.28}$} \\
\cline{2-5}
{ } & {I-DPO} & {$17.89$} &{$12.1$}&{$7.39$} \\
{ } & {+\textbf{MaPPO}} & {$\mathbf{19.84}$ $\textcolor{ForestGreen}{+1.95}$} & {$\mathbf{15.7}$ $\textcolor{ForestGreen}{+3.6}$} & {$\mathbf{7.63}$ $\textcolor{ForestGreen}{+0.24}$} \\
\midrule[1.1pt]
\multirow{5}{*}{Qwen2.5-3B-Instruct} & {IT} & {$18.91$} &{$24.0$}&{$7.92$}\\
\cline{2-5}
{ } & {DPO} & {$20.16$} &{$29.2$}&{${8.02}$} \\
{ } & {+\textbf{MaPPO}} & {$\mathbf{26.68}$ $\textcolor{ForestGreen}{+6.52}$} & {$\mathbf{35.1}$ $\textcolor{ForestGreen}{+4.9}$} & {$\mathbf{8.13}$ $\textcolor{ForestGreen}{+0.11}$} \\
\cline{2-5}
{ } & {I-DPO} & {$19.69$} &{$\mathbf{36.6}$}&{$\mathbf{8.10}$} \\
{ } & {+\textbf{MaPPO}} & {$\mathbf{25.99}$ $\textcolor{ForestGreen}{+6.30}$} & {$35.8$ $\textcolor{Apricot}{-0.8}$} & {$8.01$ $\textcolor{Apricot}{-0.09}$} \\
\midrule[1.1pt]
\multirow{5}{*}{Qwen2.5-7B-Instruct} & {IT} & {$27.03$}  & {$42.9$ }  & {$8.61$ } \\
\cline{2-5}
{ } & {DPO} & {$32.01$} &{$45.5$}&{$8.56$} \\
{ } & {+\textbf{MaPPO}} & {$\mathbf{38.24}$ $\textcolor{ForestGreen}{+6.23}$} & {$\mathbf{59.2}$ $\textcolor{ForestGreen}{+13.7}$} & {$\mathbf{8.79}$ $\textcolor{ForestGreen}{+0.23}$} \\
\cline{2-5}
{ } & {I-DPO} & {$33.80$} & {$46.9$} & {$\mathbf{8.55}$}\\
{ } & {+\textbf{MaPPO}} & {$\mathbf{39.10}$ $\textcolor{ForestGreen}{+5.30}$} & {$\mathbf{61.6}$ $\textcolor{ForestGreen}{+14.7}$} & {$8.54$ $\textcolor{Apricot}{-0.01}$}\\
\midrule[1.1pt]
\multirow{5}{*}{Mistral-7B-Instruct} & {IT}  & {$15.35$ } &{$13.1$}&{$5.40$} \\
\cline{2-5}
{ } & {DPO} & {$18.24$} &{$14.2$}&{$6.86$} \\
{ } & {+\textbf{MaPPO}} & {$\mathbf{30.56}$ $\textcolor{ForestGreen}{+12.32}$} & {$\mathbf{18.4}$ $\textcolor{ForestGreen}{+4.2}$} & {$\mathbf{7.51}$ $\textcolor{ForestGreen}{+0.65}$} \\
\cline{2-5}
{ } & {I-DPO} & {$17.11$}  & {$14.3$}  & {$6.92$} \\
{ } & {+\textbf{MaPPO}} & {$\mathbf{33.28}$ $\textcolor{ForestGreen}{+16.14}$} &{$\mathbf{19.6}$ $\textcolor{ForestGreen}{+5.3}$} & {$\mathbf{7.59}$ $\textcolor{ForestGreen}{+0.67}$}\\
\midrule[1.1pt]
\multirow{5}{*}{Llama-3-8B-Instruct} & {IT} & {$10.85$} &{$10.2$}&{$7.52$}\\
\cline{2-5}
{ } & {DPO} & {$22.48$} &{$22.4$}&{$8.07$} \\
{ } & {+\textbf{MaPPO}} & {$\mathbf{28.37}$ $\textcolor{ForestGreen}{+5.89}$} & {$\mathbf{29.5}$ $\textcolor{ForestGreen}{+7.1}$} & {$\mathbf{8.18}$ $\textcolor{ForestGreen}{+0.11}$} \\
\cline{2-5}
{ } & {I-DPO} & {${29.47}$} &{$25.6$ }&{$8.01$}\\
{ } & {+\textbf{MaPPO}} & {$\mathbf{32.68}$ $\textcolor{ForestGreen}{+3.21}$} & {$\mathbf{31.0}$ $\textcolor{ForestGreen}{+5.4}$} & {$\mathbf{8.04}$ $\textcolor{ForestGreen}{+0.03}$} \\
\bottomrule[1.1pt]
\end{tabular}
\end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Adaptation to DPO Variants}
\label{sec:adapt}

In Table \ref{table:adaptation}, we show the improvement of the vanilla DPO~\citep{dpo_neurips2023} and its variants with MaPPO, including widely used I-DPO~\citep{dong2024rlhf}, SimPO~\citep{meng2024simpo}, IPO~\citep{pmlr-v238-gheshlaghi-azar24a}, and CPO~\citep{xu2024contrastive}. 
We list the hyperparameter settings in the DPO variants in Appendix \ref{app:Experiments}. 
Their loss functions with MaPPO adaptation are shown in Section \ref{sec:online_mappo} and Section \ref{sec:adapt_other_po}. 
For all DPO variants, no additional hyperparameter is needed from the MaPPO plugin. For the model in evaluation, we keep Qwen2.5-7B-Instruct as the default model. 

In general, MaPPO consistently improves all DPO variants with the MLE design on all three benchmarks.
% The model achieves the highest performance with MaPPO in the online setting on I-DPO. 
Although it drops a little on MT-Bench in some methods, the original approach has essentially saturated at the achievable score on MT-Bench, which barely reflects the improvement with a variance in evaluation.
The overall consistent improvements observed across DPO variants after applying the MaPPO plugin underscore its flexibility and generality in enhancing preference optimization methods. 
Notably, MaPPO effectively complements both simple and complex variants without requiring architectural modifications or hyperparameter tuning. 
For instance, SimPO benefits from the MaPPO adjustment by further balancing the length-controlled optimization with better calibration of confidence scores, while IPO and CPO experience gains due to MaPPO’s capacity to regularize reward signals with prior knowledge, mitigating overfitting to pairwise preferences. 
The improvements span diverse evaluation metrics and benchmarks, demonstrating that MaPPO’s reward-aware calibration systematically addresses the shortcomings of MLE-based objectives inherent in existing variants. 
This indicates that MaPPO is not merely a tweak, but a general principle that can be seamlessly integrated into the PO pipelines to achieve more reliable alignment results.

\begin{table}[!ht]
\caption{Evaluation results of DPO variants with a MaPPO plugin. $\uparrow$ indicates the higher the better.}
\centering
 % \small
\label{table:adaptation}
\begin{tabular}{l|lll}
\toprule[1.1pt]
% \hline
{Method} & {AlpacaEval 2.0 $\uparrow$} & {Arena-Hard $\uparrow$} & {MT-Bench $\uparrow$} \\
\midrule[1.1pt]
{DPO~\citep{dpo_neurips2023}} & {$32.01$} &{$45.5$}&{$8.56$} \\
{+\textbf{MaPPO}} & {$\mathbf{38.24}$ $\textcolor{ForestGreen}{+6.23}$} & {$\mathbf{59.2}$ $\textcolor{ForestGreen}{+13.7}$} & {$\mathbf{8.79}$ $\textcolor{ForestGreen}{+0.23}$} \\
\cline{1-4}
{I-DPO~\citep{dong2024rlhf}} & {$33.80$} &{$46.9$}&{$\mathbf{8.55}$} \\
{+\textbf{MaPPO}} & {$\mathbf{39.10}$ $\textcolor{ForestGreen}{+5.30}$} & {$\mathbf{61.6}$ $\textcolor{ForestGreen}{+14.7}$} & {$8.54$ $\textcolor{Apricot}{-0.01}$} \\
\cline{1-4}
{SimPO~\citep{meng2024simpo}} & {$25.15$} &{$64.2$}&{$\mathbf{9.02}$} \\
{+\textbf{MaPPO}} & {$\mathbf{32.75}$ $\textcolor{ForestGreen}{+7.60}$} & {$\mathbf{69.5}$ $\textcolor{ForestGreen}{+5.3}$} & {${8.94}$ $\textcolor{Apricot}{-0.08}$} \\
\cline{1-4}
{IPO~\citep{pmlr-v238-gheshlaghi-azar24a}} & {$27.76$} &{$53.0$}&{$8.83$} \\
{+\textbf{MaPPO}} & {$\mathbf{28.84}$ $\textcolor{ForestGreen}{+1.08}$} & {$\mathbf{64.4}$ $\textcolor{ForestGreen}{+11.4}$} & {$\mathbf{8.84}$ $\textcolor{ForestGreen}{+0.01}$} \\
\cline{1-4}
{CPO~\citep{xu2024contrastive}} & {$32.94$} &{$47.6$}&{8.62} \\
{+\textbf{MaPPO}} & {$\mathbf{33.71}$ $\textcolor{ForestGreen}{+0.77}$} & {$\mathbf{54.1}$ $\textcolor{ForestGreen}{+6.5}$} & {$\mathbf{8.68}$ $\textcolor{ForestGreen}{+0.06}$} \\
\bottomrule[1.1pt]
\end{tabular}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Other Results on Academic Benchmarks}

It is widely observed that alignment impairs models' performance on calibration, reasoning, and accuracy \citep{ouyang2022training, LinL0DLZP00ZDPZ24, zhang2025iterative}, which is also known as the alignment tax. As a result, it is also needed to assess the model’s performance using more academic benchmarks. In this subsection, we investigate whether the serval methods for alignment with human preference could sacrifice the general model performance.

We test the performance on six widely used academic benchmarks, evaluating various model abilities, including explicit instruction following (IFEval) \citep{zhou2023instruction}, general knowledge (GPQA) \citep{rein2024gpqa}, multitask language understanding (MMLU) \citep{hendrycks2021measuring}, commonsense reasoning (HellaSwag) \citep{zellers-etal-2019-hellaswag}, human falsehoods mimicking (TruthfulQA) \citep{lin-etal-2022-truthfulqa}, and math word problem-solving (GSM8K) \citep{cobbe2021training}. 

We show the results on the six academic benchmarks from Llama-3-8B-Instruct model in Table \ref{table:academic}, and Qwen2.5-7B-Instruct model in Table \ref{table:academic_qwen_7b}. In general, for offline DPO with MaPPO outperforms the original DPO in all benchmarks for both models. The improvement is significant on GSM8K for Qwen2.5-7B-Instruct, and on TruthfulQA for Llama-3-8B-Instruct. For the iterative DPO with MaPPO, the performances are better than the original I-DPO on most benchmarks, and maintains the performances on IFEval and GPQA. Overall, the performances of online methods are better than offline methods, and MaPPO generally improves or maintains the  performances on academic benchmarks in both settings.

\begin{table}[!ht]
\vspace{-4mm}
\caption{Evaluation results on six academic benchmarks with Llama-3-8B-Instruct model.}
\centering
 % \small
\label{table:academic}
\begin{tabular}{l|cccccc}
\toprule[1.1pt]
% \hline
 {Method} & {IFEval $\uparrow$} & {GPQA $\uparrow$} & {MMLU $\uparrow$} & {HellaSwag $\uparrow$} & {TruthfulQA $\uparrow$} & {GSM8K $\uparrow$} \\
\midrule[1.1pt]
{IT} & {$70.4$} & {$30.2$} & {$62.4$} & {$78.6$} & {$53.7$} & {$73.4$} \\
\hline
{DPO} & {$77.0$} & {$27.5$} & {$62.7$} & {$79.5$} & {$51.5$} & {$75.5$}  \\
{+\textbf{MaPPO}} & {$\mathbf{82.0}$} & {$\mathbf{29.5}$} & {$\mathbf{63.2}$} & {$\mathbf{80.1}$} & {$\mathbf{58.2}$} 
& {$\mathbf{79.5}$} \\
\hline
{I-DPO} & {$74.6$} & {$\mathbf{29.8}$} & {$63.1$} & {$80.5$} & {$60.7$} & {$81.3$} \\
{+\textbf{MaPPO}} & $\mathbf{76.4}$ & ${28.8}$ & $\mathbf{63.5}$ & $\mathbf{80.7}$ & $\mathbf{63.7}$ & $\mathbf{82.4}$ \\
\bottomrule[1.1pt]
\end{tabular}
\end{table}
\begin{table}[!ht]
\caption{Evaluation results on six academic benchmarks with Qwen2.5-7B-Instruct model.}
\centering
 % \small
\label{table:academic_qwen_7b}
\begin{tabular}{l|cccccc}
\toprule[1.1pt]
% \hline
 {Method} & {IFEval $\uparrow$} & {GPQA $\uparrow$} & {MMLU $\uparrow$} & {HellaSwag $\uparrow$} & {TruthfulQA $\uparrow$} & {GSM8K $\uparrow$} \\
\midrule[1.1pt]
{IT} & {$73.5$} & {$31.5$} & {$71.8$} & {$62.1$} & {$56.4$} & {$81.7$} \\
\hline
{DPO} & {$73.2$} & {$32.0$} & {$71.9$} & {$62.0$} & {$57.1$} & {$71.3$}  \\
{+\textbf{MaPPO}} & {$\mathbf{73.8}$} & {$\mathbf{33.1}$} & {$\mathbf{72.0}$} & {$\mathbf{62.1}$} & {$\mathbf{59.2}$} 
& {$\mathbf{80.1}$} \\
\hline
{I-DPO} & {$\textbf{72.9}$} & {$33.0$} & {$71.9$} & {$62.2$} & {$55.9$} & {$73.2$} \\
{+\textbf{MaPPO}} & $72.6$ & ${\textbf{33.3}}$ & $\mathbf{72.9}$ & $\mathbf{62.2}$ & $\mathbf{56.2}$ & $\mathbf{82.0}$ \\
\bottomrule[1.1pt]
\end{tabular}
\end{table}

% \begin{table}[!ht]
% \caption{Evaluation results on academic benchmarks with LLaMA-3-8B-Instruct model.}
% \centering
%  % \small
% \label{table:academic_LLaMA-3-8B-Ins}
% \begin{tabular}{c|cccccc}
% \toprule[1.1pt]
% % \hline
%  {Method} & {IFEval} & {GPQA} & {MMLU} & {HellaSwag} & {TruthfulQA} & {GSM8K} \\
% \midrule[1.1pt]
% {SFT} & { } & { } & { } & { } & { } & { } \\
% {DPO} & { } & { } & { } & { } & { } & { } \\
% {I-DPO} & { } & { } & { } & { } & { } & { } \\
% {IPO} & { } & { } & { } & { } & { } & { } \\
% {ORPO} & { } & { } & { } & { } & { } & { } \\
% {KTO} & { } & { } & { } & { } & { } & { } \\
% {\textbf{MaPPO}} & { } & { } & { } & { } & { } & { } \\
% \bottomrule[1.1pt]
% \end{tabular}
% \end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Discussions}
\label{Sec:Discussions}

\subsection{Summary}

In this chapter, we introduced Maximum a Posteriori Preference Optimization (MaPPO), a general preference-optimization framework that incorporates prior reward knowledge into the optimization objective. By extending the conventional maximum-likelihood formulation of preference optimization to a Maximum a Posteriori formulation, MaPPO provides a more calibrated training signal and mitigates confidence degeneration during alignment. The method supports both offline and online settings, requires no additional hyperparameters, and can be integrated naturally with existing DPO-style methods, including SimPO, IPO, and CPO. Extensive empirical results showed that MaPPO consistently improves alignment performance across multiple model families, model sizes, and standard benchmarks, while maintaining strong performance on broader academic evaluations. These results suggest that prior-informed preference optimization is a promising direction for improving the reliability and effectiveness of LLM alignment.

\subsection{Limitations and Future Work}

Despite the strong empirical performance of MaPPO, several limitations remain.

First, the current results indicate that larger models tend to benefit more consistently from the MaPPO framework. Future work with greater computational resources could study the behavior of the proposed method on substantially larger language models.

Second, the design of the prior knowledge function still depends on domain knowledge. While the current design is general and effective, future work could investigate more adaptive, data-driven, or theoretically grounded prior-function designs for specific application domains or preference structures.

Third, the present evaluation primarily relies on benchmark-based automatic assessment. More extensive human evaluation would provide a more direct understanding of whether the improved training signal translates into more desirable real-world alignment behavior.

Finally, a promising broader direction is to study tighter integration between prior-informed preference optimization and other reinforcement-learning-based post-training methods, including settings in which preference data, reward signals, and online rollouts are jointly refined during training.

==> papers/mappo/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak
